Soft regression trees: a model variant and a decomposition training algorithm

Decision trees are widely used for classification and regression tasks in a variety of application fields due to their interpretability and good accuracy. During the past decade, growing attention has been devoted to globally optimized decision trees with deterministic or soft splitting rules at branch nodes, which are trained by optimizing the error function over all the tree parameters. In this work, we propose a new variant of soft multivariate regression trees (SRTs) where, for every input vector, the prediction is defined as the linear regression associated to a single leaf node, namely, the leaf node obtained by routing the input vector from the root along the branches with higher probability. SRTs exhibit the conditional computational property, i.e., each prediction depends on a small number of nodes (parameters), and our nonlinear optimization formulation for training them is amenable to decomposition. After showing a universal approximation result for SRTs, we present a decomposition training algorithm including a clustering-based initialization procedure and a heuristic for reassigning the input vectors along the tree. Under mild assumptions, we establish asymptotic convergence guarantees. Experiments on 15 wellknown datasets indicate that our SRTs and decomposition algorithm yield higher accuracy and robustness compared with traditional soft regression trees trained using the nonlinear optimization formulation of Blanquero et al., and a significant reduction in training times as well as a slightly better average accuracy compared with the mixed-integer optimization approach of Bertsimas and Dunn. We also report a comparison with the Random Forest ensemble method.

==> sections/experiment_old.tex <==
\section{Experimental results}\label{sec.experiments}

In this section we assess the performance of the regression tree training methodology, consisting in solving formulation \ref{eq:obj} by means of decomposition algorithm \ref{alg:Decomposition1}. Such methodology is referred to as MRRT. The section is organized as follows. Subsection \ref{sec:dataset_exp} describes the experimental settings and the datasets. In Subsection \ref{sec:results_exp} we compare the prediction accuracy of MRRT with several benchmark methods for building regression trees.

\subsection{Datasets and experimental setting}
\label{sec:dataset_exp}
In this subsection we present the datasets and describe the experimental setting. We consider 15 well-known datasets from the UCI Machine Learning Repository \cite{} and the KEEL repository \cite{}. Table \ref{tab:dataset} reports a description of the 15 datasets.

\begin{table}[h]
\caption{The description of the 15 datasets.} \label{tab:dataset}
\centering
\renewcommand{\arraystretch}{0.7}
\resizebox{0.4\columnwidth}{!}{
\begin{tabular}{lllllll}
\hline
\multicolumn{1}{c}{Dataset} &  & \multicolumn{1}{c}{Abbreviation} &  & \multicolumn{1}{c}{N} &  & \multicolumn{1}{c}{p} \\ \hline
Abalone                     &  & Abalone                          &  & 4177                  &  & 8                     \\
Ailerons                    &  & Ailerons                         &  & 7154                  &  & 40                    \\
Airfoil                     &  & Airfoil                          &  & 1503                  &  & 5                     \\
Auto mpg                    &  & Auto                          &  & 392                   &  & 7                     \\
Compactiv                     &  & Compact                          &  & 8192                  &  & 21                    \\
Computer hardware           &  & Computer                         &  & 209                   &  & 37                    \\
Cpu small                   &  & Cpu small                        &  & 8192                  &  & 12                    \\
Delta ailerons              &  & Delta                    &  & 7129                  &  & 5                     \\
Elevators                   &  & Elevators                        &  & 16599                 &  & 18                    \\
Friedman artificial         &  & Friedman                         &  & 40768                 &  & 10                    \\
Housing                     &  & Housing                          &  & 506                   &  & 13                    \\
Kin8nm                      &  & Kin8nm                           &  & 8192                  &  & 8                     \\
Lpga2009                        &  & Lpga2009                             &  & 146                  &  & 11                    \\
Puma                        &  & Puma                             &  & 8192                  &  & 32                    \\
Yacht hydrodynamics         &  & Yacht                            &  & 308                   &  & 6                     \\ \hline
\end{tabular}
}
\end{table}

To assess the testing accuracy we use the testing R squared:
$R^2 = 1 - \frac{SS_{res}^{test}}{SS_{tot}^{test}}$
where $SS_{res}^{test}$ is the sum of squares of residuals and $SS_{tot}^{test}$ is the total sum of squares, both on testing data points. The testing $R^2$ are evaluated by means of $k$-fold cross-validation, with $k= 4$. 
Each dataset is randomly divided into $k$  %subsamples 
subsets of samples.  
In turn, every subset of samples is considered as testing set, while the rest is used to train the model. Therefore, all the samples are used both for training and testing.
Then the model accuracy is computed as the average of the accuracies obtained over all $k$ folds. 
For each fold the model is trained with $20$ different random seeds used to generate different starting points with the initialization strategy. The final testing $R^2$ is the average of the $R^2$ over the $80$ trained models. 

%The experiments are carried out on a PC with Intel(R) Core(TM) i7-9700K CPU @ 3.60GHz with 16GB RAM. The MRRT formulation have been implemented in Python 3.6. For the optimization of the leaf nodes variables we used \texttt{scipy.sparse.linalg.lsqr} in the scipy sparse linear algebra package  \texttt{scipy.sparse}. For the optimization of the branching nodes variables, in the case of generic optimization, we use the SLSQP solver in \texttt{scipy.optimize} package in tandem with \texttt{numba} while for the balanced logistic regression we used the logistic regression model from  \texttt{sklearn} package. we find the least-squares solution by means of the command \texttt{scipy.sparse.linalg.lsqr} in the scipy sparse linear algebra package  \texttt{scipy.sparse}. In the case of the $l_0$ concave approximation we use the SLSQP solver in \texttt{scipy.optimize} package in tandem with \texttt{numba} 


\subsection{Comparative results}
\label{sec:results_exp}
The MRRT methodology is evaluated in two different versions: with and without $\ell_2$ regularization term included into the loss function \eqref{eq:obj}, which, for simplicity, are denoted as MRRT $\ell_2$ and MRRT, respectively. For the the MRRT $\ell_2$ the regularization terms $\lambda_{\bm{\w}}$ and $\lambda_{\bm{\beta}}$ are set as $\lambda_{\bm{w}}=\frac{2}{p \times |\tau_{B}|}$ and $\lambda_{\bm{\beta}}=\frac{2}{p \times |\tau_{L}|}$. Such versions are compared with two alternative regression tree training methodologies. 

The first one is Optimal Regression Tree with Linear predictions (ORT-L) proposed in \cite{dunn2018optimal,bertsimas2019machine}, which is based on solving a MILP formulation by means of a local search heuristic. In particular, ORT-L constructs deterministic univariate regression trees that involve linear predictions with Lasso sparsity terms at each leaf node. In the same work the authors also proposed a more general and computational demanding version of ORT-L involving hyperplane splits, and denoted as ORT-LH. However, the experimental results on three datasets reported in Appendix \ref{appendix:ortl_vs_ortlh} show that the large increase in computational time of ORT-LH is not compensated by a significant $R^2$ improvement. It is worth pointing out that the fact that ORT-L and ORT-LH provide comparable $R^2$ was already highlighted in the experiments in \cite{dunn2018optimal,bertsimas2019machine}. 

The second methodology is Optimal Randomized Regression Tree (ORRT) proposed in \cite{blanquero2021sparse}, which is based on solving a nonlinear continuous formulation. \textcolor{blue}{
It is important to point out that in \cite{blanquero2021sparse} the authors adopt as evaluation criterion a multistart approach, namely the best solution found over a prescribed number o starting points is returned. Unlike in \cite{blanquero2021sparse}, our criterion involves calculating the average performance measures across all starting points and k-folds. This widely used criterion, which involves considering the average over multiple starting points and k-folds, provides a more comprehensive and reliable assessment of the expected performance of the model. To illustrate the possible impact of the two evaluation criteria on ORRT performance, experimental results obtained on four datasets are reported in Appendix \ref{appendix:orrt_multi}.}


\begin{table}[]
\centering
\caption{Comparison between MRRT, MRRT $l_2$, ORT-L and ORRT with depth $D = 2$. Anomaly corresponds to solutions with negative out-of-sample $R^2$. The number of negative $R^2$ for MRRT, MRRT $l_2$ and ORT-L is equal to 0.}\label{tab:depth2}
\resizebox{\textwidth}{!}{\begin{tabular}{lccccccccccccccc}
\hline
                               & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}    & \multicolumn{13}{c}{D=2}                                                                                                                                                                                                                                                                 \\ \cline{4-16} 
\multicolumn{3}{c}{}                                                            & \multicolumn{3}{c}{MRRT}                           & \multicolumn{3}{c}{MRRT $l_2$}                     & \multicolumn{3}{c}{ORT L}                            & \multicolumn{4}{c}{ORRT}                                                                                                \\ \cline{4-16} 
Dataset                        & N                    & p                       & $R^2$ & \multicolumn{1}{c}{$\sigma${\tiny ($1e^{-2}$)}} & \multicolumn{1}{c}{Time}                        & $R^2$ & \multicolumn{1}{c}{$\sigma${\tiny ($1e^{-2}$)}} & \multicolumn{1}{l}{Time}                        & \multicolumn{1}{c}{$R^2$} & \multicolumn{1}{c}{$\;\;\;\sigma${\tiny ($1e^{-2}$)}} & \multicolumn{1}{c}{Time}      & \multicolumn{1}{c}{$R^2$} & \multicolumn{1}{c}{$\sigma${\tiny ($1e^{-2}$)}} & \multicolumn{1}{c}{Time} & \multicolumn{1}{l}{$R^2<0$} \\ \hline
\multicolumn{1}{l|}{Abalone}   & 4177                 & \multicolumn{1}{c|}{8}  & 0.551 & 2.18         & \multicolumn{1}{c|}{8.59}   & 0.554 & 2.14         & \multicolumn{1}{c|}{8.74}   & 0.558 & 1.7          & \multicolumn{1}{c|}{70.62}    & 0.525                     & 3.32                             & 18.17                    & 8                             \\
\multicolumn{1}{l|}{Ailerons}  & 7154                 & \multicolumn{1}{c|}{40} & 0.833 & 0.6          & \multicolumn{1}{c|}{18.99}  & 0.836 & 0.56         & \multicolumn{1}{c|}{18.95}  & 0.824 & 1.13         & \multicolumn{1}{c|}{262.16}   & 0.771                     & 13.53                            & 427.73                   & 45                            \\
\multicolumn{1}{l|}{Airfoil}   & 1503                 & \multicolumn{1}{c|}{5}  & 0.762 & 3.15         & \multicolumn{1}{c|}{5.21}   & 0.748 & 2.9          & \multicolumn{1}{c|}{5.16}   & 0.744 & 1.6          & \multicolumn{1}{c|}{2.07}     & 0.516                     & 2.89                             & 1.81                     & 4                             \\
\multicolumn{1}{l|}{Auto mpg}  & 392                  & \multicolumn{1}{c|}{7}  & 0.853 & 2            & \multicolumn{1}{c|}{2.48}   & 0.87  & 2.37         & \multicolumn{1}{c|}{2.47}   & 0.838 & 2.8          & \multicolumn{1}{c|}{5.94}     & 0.811                     & 2.23                             & 0.89                     & 17                            \\
\multicolumn{1}{l|}{Compact}   & 8192                 & \multicolumn{1}{c|}{21} & 0.979 & 0.25         & \multicolumn{1}{c|}{35.47}  & 0.98  & 0.168        & \multicolumn{1}{c|}{37.17}  & 0.981 & 0.34         & \multicolumn{1}{c|}{668.37}   & 0.692                     & 13.1                             & 183.2                    & 11                            \\
\multicolumn{1}{l|}{Computer}  & 209                  & \multicolumn{1}{c|}{37} & 0.977 & 1.86         & \multicolumn{1}{c|}{1.97}   & 0.964 & 2.49         & \multicolumn{1}{c|}{1.99}   & 0.877 & 13.4         & \multicolumn{1}{c|}{1.9}      & 0.907                     & 5.5                              & 0.572                    & 10                            \\
\multicolumn{1}{l|}{Cpu small} & 8192                 & \multicolumn{1}{c|}{12} & 0.969 & 0.32         & \multicolumn{1}{c|}{33.78}  & 0.969 & 0.23         & \multicolumn{1}{c|}{31.34}  & 0.97  & 0.24         & \multicolumn{1}{c|}{215.09}   & 0.72                      & 4                                & 62.65                    & 6                             \\
\multicolumn{1}{l|}{Delta}     & 7129                 & \multicolumn{1}{c|}{5}  & 0.701 & 0.64         & \multicolumn{1}{c|}{10.96}  & 0.701 & 0.63         & \multicolumn{1}{c|}{10.4}   & 0.697 & 0.7          & \multicolumn{1}{c|}{7.577}    & 0.678                     & 0.7                              & 8.56                     & 4                             \\
\multicolumn{1}{l|}{Elevators} & 16599                & \multicolumn{1}{c|}{18} & 0.872 & 0.5          & \multicolumn{1}{c|}{40.69}  & 0.871 & 0.47         & \multicolumn{1}{c|}{39.55}  & 0.812 & 0.58         & \multicolumn{1}{c|}{482.6}    & 0.813                     & 0.6                              & 220.37                   & 26                            \\
\multicolumn{1}{l|}{Friedman}  & 40768                & \multicolumn{1}{c|}{10} & 0.895 & 0.75         & \multicolumn{1}{c|}{134.34} & 0.894 & 0.85         & \multicolumn{1}{c|}{134.46} & 0.886 & 0.13         & \multicolumn{1}{c|}{294.2}    & 0.723                     & 0.18                             & 56.28                    & 6                             \\
\multicolumn{1}{l|}{Housing}   & 506                  & \multicolumn{1}{c|}{13} & 0.85  & 4.6          & \multicolumn{1}{c|}{2.94}   & 0.846 & 3.4          & \multicolumn{1}{c|}{2.92}   & 0.782 & 5.17         & \multicolumn{1}{c|}{43.49}    & 0.699                     & 10.4                             & 3.8                      & 7                             \\
\multicolumn{1}{l|}{Kin8nm}    & 8192                 & \multicolumn{1}{c|}{8}  & 0.72  & 1.9          & \multicolumn{1}{c|}{19.62}  & 0.723 & 2.28         & \multicolumn{1}{c|}{19.02}  & 0.566 & 1.8          & \multicolumn{1}{c|}{439.79}   & 0.412                     & 1.2                              & 10.95                    & 5                             \\
\multicolumn{1}{l|}{Lpga2009}  & 146                  & \multicolumn{1}{c|}{11} & 0.765 & 7.4          & \multicolumn{1}{c|}{2.23}   & 0.891 & 2.58         & \multicolumn{1}{c|}{2.23}   & 0.86  & 3.1          & \multicolumn{1}{c|}{12.11}    & 0.864                     & 10.9                             & 0.89                     & 4                             \\
\multicolumn{1}{l|}{Puma}      & 8192                 & \multicolumn{1}{c|}{32} & 0.815 & 0.96         & \multicolumn{1}{c|}{45.31}  & 0.815 & 0.9          & \multicolumn{1}{c|}{44.95}  & 0.823 & 0.9          & \multicolumn{1}{c|}{10592.25} & 0.216                     & 3.2                              & 53.54                    & 7                             \\
\multicolumn{1}{l|}{Yacht}     & 308                  & \multicolumn{1}{c|}{6}  & 0.987 & 0.58         & \multicolumn{1}{c|}{2.54}   & 0.976 & 0.77         & \multicolumn{1}{c|}{2.49}   & 0.991 & 0.18         & \multicolumn{1}{c|}{0.972}    & 0.643                     & 6.2                              & 0.636                    & 11                            \\ \hline
\multicolumn{3}{c}{AVG ARIT}                                                    & 0.835 & 1.85         & \multicolumn{1}{c|}{24.34}  & 0.843 & 1.5          & \multicolumn{1}{c|}{24.12}  & 0.814 & 2.25         & \multicolumn{1}{c|}{873.27}   & 0.666                     & 5.2                              & 70.0                     &                               \\ \hline
\multicolumn{3}{c}{AVG GEOM}                                                    & 0.827 & 1.2          & \multicolumn{1}{c|}{11.6}   & 0.834 & 1.07         & \multicolumn{1}{c|}{11.48}  & 0.804 & 1.11         & \multicolumn{1}{c|}{66.3}     & 0.635                     & 3.14                             & 13.12                    &                               \\ \hline
\end{tabular}
}
\end{table}



\begin{table}[]
\caption{Comparison between MRRT, MRRT $l_2$, ORT-L and ORRT with depth $D = 3$. Anomaly corresponds to solutions with negative out-of-sample $R^2$. The number of negative $R^2$ for MRRT, MRRT $l_2$ and ORT-L is equal to 0.}\label{tab:depth3}
\centering
\resizebox{\textwidth}{!}{\begin{tabular}{lccccccccccccccc}
\hline
                               & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}    & \multicolumn{13}{c}{D=3}                                                                                                                                                                                   \\ \cline{4-16} 
                               & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}    & \multicolumn{3}{c}{MRRT}                           & \multicolumn{3}{c}{MRRT $l_2$}                     & \multicolumn{3}{c}{ORT L}                           & \multicolumn{4}{c}{ORRT}                   \\ \cline{4-16} 
Dataset                        & N                    & p                       & $R^2$ & \multicolumn{1}{c}{$\sigma${\tiny ($1e^{-2}$)}} & Time                        & $R^2$ & \multicolumn{1}{c}{$\sigma${\tiny ($1e^{-2}$)}} & Time                        & $R^2$ & \multicolumn{1}{c}{$\sigma${\tiny ($1e^{-2}$)}} & Time                         & $R^2$ & \multicolumn{1}{c}{$\sigma${\tiny ($1e^{-2}$)}} & Time    & $R^2<0$ \\ \hline
\multicolumn{1}{l|}{Abalone}   & 4177                 & \multicolumn{1}{c|}{8}  & 0.558 & 2.67         & \multicolumn{1}{c|}{24.55}  & 0.564 & 2.16         & \multicolumn{1}{c|}{23.97}  & 0.545 & 1.9          & \multicolumn{1}{c|}{147.98}  & 0.516 & 6.67         & 107.59  & 20        \\
\multicolumn{1}{l|}{Ailerons}  & 7154                 & \multicolumn{1}{c|}{40} & 0.826 & 0.9          & \multicolumn{1}{c|}{50.62}  & 0.835 & 0.43         & \multicolumn{1}{c|}{50.48}  & 0.825 & 1.2          & \multicolumn{1}{c|}{310.49}  & 0.784 & 11.65        & 2491.85 & 44        \\
\multicolumn{1}{l|}{Airfoil}   & 1503                 & \multicolumn{1}{c|}{5}  & 0.816 & 3.9          & \multicolumn{1}{c|}{11.23}  & 0.807 & 2.14         & \multicolumn{1}{c|}{11.35}  & 0.842 & 1.3          & \multicolumn{1}{c|}{4.69}    & 0.513 & 1.8          & 9.04    & 20        \\
\multicolumn{1}{l|}{Auto mpg}  & 392                  & \multicolumn{1}{c|}{7}  & 0.842 & 4.12         & \multicolumn{1}{c|}{6.18}   & 0.873 & 2.17         & \multicolumn{1}{c|}{6.15}   & 0.819 & 6.47         & \multicolumn{1}{c|}{10.02}   & 0.815 & 2.45         & 6.81    & 7         \\
\multicolumn{1}{l|}{Compact}   & 8192                 & \multicolumn{1}{c|}{21} & 0.979 & 0.38         & \multicolumn{1}{c|}{72.13}  & 0.98  & 0.27         & \multicolumn{1}{c|}{72.72}  & 0.98  & 0.48         & \multicolumn{1}{c|}{1103.46} & 0.721 & 3.4          & 905.65  & 5         \\
\multicolumn{1}{l|}{Computer}  & 209                  & \multicolumn{1}{c|}{37} & 0.973 & 1.8          & \multicolumn{1}{c|}{4.02}   & 0.955 & 3.37         & \multicolumn{1}{c|}{4.03}   & 0.889 & 16           & \multicolumn{1}{c|}{3.2}     & 0.887 & 13.8         & 4.27    & 14        \\
\multicolumn{1}{l|}{Cpu small} & 8192                 & \multicolumn{1}{c|}{12} & 0.969 & 0.26         & \multicolumn{1}{c|}{57.19}  & 0.97  & 0.25         & \multicolumn{1}{c|}{58.67}  & 0.971 & 0.31         & \multicolumn{1}{c|}{427.41}  & 0.705 & 7.24         & 323.2   & 3         \\
\multicolumn{1}{l|}{Delta}     & 7129                 & \multicolumn{1}{c|}{5}  & 0.704 & 1.11         & \multicolumn{1}{c|}{28.4}   & 0.706 & 1            & \multicolumn{1}{c|}{29.53}  & 0.709 & 0.77         & \multicolumn{1}{c|}{17.38}   & 0.672 & 2.7          & 52.68   & 4         \\
\multicolumn{1}{l|}{Elevators} & 16599                & \multicolumn{1}{c|}{18} & 0.886 & 0.52         & \multicolumn{1}{c|}{97.64}  & 0.884 & 0.57         & \multicolumn{1}{c|}{94.66}  & 0.812 & 0.58         & \multicolumn{1}{c|}{515.78}  & 0.783 & 10.3         & 1476.75 & 21        \\
\multicolumn{1}{l|}{Friedman}  & 40768                & \multicolumn{1}{c|}{10} & 0.937 & 0.53         & \multicolumn{1}{c|}{310.47} & 0.938 & 0.28         & \multicolumn{1}{c|}{311.76} & 0.935 & 0.06         & \multicolumn{1}{c|}{1356.56} & 0.721 & 1.23         & 455.75  & 13        \\
\multicolumn{1}{l|}{Housing}   & 506                  & \multicolumn{1}{c|}{13} & 0.809 & 8.3          & \multicolumn{1}{c|}{7.23}   & 0.872 & 4.48         & \multicolumn{1}{c|}{7.35}   & 0.785 & 8.3          & \multicolumn{1}{c|}{78.4}    & 0.715 & 6.1          & 19.14   & 10        \\
\multicolumn{1}{l|}{Kin8nm}    & 8192                 & \multicolumn{1}{c|}{8}  & 0.787 & 1.9          & \multicolumn{1}{c|}{50.18}  & 0.786 & 1.9          & \multicolumn{1}{c|}{50.73}  & 0.645 & 1.1          & \multicolumn{1}{c|}{946.47}  & 0.412 & 1            & 45.9    & 9         \\
\multicolumn{1}{l|}{Lpga2009}  & 146                  & \multicolumn{1}{c|}{11} & 0.8   & 11.3         & \multicolumn{1}{c|}{4.92}   & 0.877 & 2.5          & \multicolumn{1}{c|}{4.96}   & 0.844 & 4            & \multicolumn{1}{c|}{16.53}   & 0.88  & 4.2          & 4.58    & 8         \\
\multicolumn{1}{l|}{Puma}      & 8192                 & \multicolumn{1}{c|}{32} & 0.884 & 0.91         & \multicolumn{1}{c|}{135.93} & 0.883 & 0.88         & \multicolumn{1}{c|}{136.51} & 0.907 & 0.39  &  \multicolumn{1}{c|}{28481.81}        & 0.215 & 3.2          & 233.07  & 13        \\
\multicolumn{1}{l|}{Yacht}     & 308                  & \multicolumn{1}{c|}{6}  & 0.99  & 0.49         & \multicolumn{1}{c|}{5.18}   & 0.983 & 0.48         & \multicolumn{1}{c|}{5.41}   & 0.992 & 0.11         & \multicolumn{1}{c|}{2.81}    & 0.645 & 5.6          & 3.57    & 21        \\ \hline
\multicolumn{3}{c}{AVG ARIT}                                                    & 0.851 & 2.6          & \multicolumn{1}{c|}{57.72}  & 0.861 & 1.52         & \multicolumn{1}{c|}{57.88}  & 0.833     & 2.87            & \multicolumn{1}{c|}{2228.2}       & 0.666 & 5.42         & 409.32  &           \\ \hline
\multicolumn{3}{c}{AVG GEOM}                                                    & 0.843 & 1.46         & \multicolumn{1}{c|}{27.19}  & 0.853 & 1.05         & \multicolumn{1}{c|}{27.38}  & 0.823     & 1.02            & \multicolumn{1}{c|}{109.48}       & 0.635 & 4.22         & 75.0    &           \\ \hline
\end{tabular}
}
\end{table}




\textcolor{blue}{The numerical experiments are carried out for tree models of depth $D=2$ in Table \ref{tab:depth2} and of depth $D=3$ in Table \ref{tab:depth3}. For each method the tables show the average out-of-sample $R^2$, its standard deviation $\sigma$ (divided by a $1e^{-2}$ factor for visualization reasons) and the average training time. For the ORRT model we also indicate the negative $R^2$ column, which represents the number of times that the training phase crushs in a suboptimal solution with a negative testing $R^2$. For each dataset the bold indicates that the method is the best in terms of testing $R^2$. At the bottom of the tables the arithmetic and the geometric averages $R^2$ across all datasets are reported.}


\textcolor{blue}{Overall, as shown in the last rows containing the average results, for both depths MRRT $l_2$ is the best in terms of out-of-sample $R^2$, $\sigma$, and computational time. Since for both depths the results are qualitatively similar, we focus our discussion on the results obtained at depth $D=3$ which presents a more challenging and complex problem, thus offering greater interest for analysis.}



\textcolor{blue}{In the comparison between the two alternative MRRTs, the last two rows in Table \ref{tab:depth3} illustrate how for the same computational time and $\sigma$, MRRTs with $l_2$ regularization exhibit slightly better performance in terms of out-of-sample $R^2$, with an improvement of approximately $1\%$. This suggests that the inclusion of $l_2$ regularization term enhances the robustness of the models, and this is quite evident by looking at the results for datasets such as lpga2009 and housing, where the MRRTs $l_2$ outperform its counterpart by more than $6\%$.}

\textcolor{blue}{Concerning the comparison between the ORRT and MRRT $l_2$, the MRRT $l_2$ outperform the ORRT in terms of $R^2$, with a gap of more than $18\%$ on average and a smaller standard deviation, thus solutions less sensitive with respect to starting points. Moreover, computational times are favorable to the MRRT $l_2$ with a good reduction with respect to the time required by ORRT (about one-seventh on arithmetic average and one-third on geometric average).}

\textcolor{blue}{For example, in datasets such as kin8nm or Yacht there is a difference of more than $30\%$ in $R^2$ for the same computational time, while in the case of the Puma dataset there is a difference of more than $60\%$ for twice the computational time required. Another example is the compact dataset where against a difference of over $25\%$ in favor of MRRT $l_2$, the ORRT model requires over 12 times more computational time. It is interesting to note the result of the lpga2009 dataset where ORRT manages to obtain a slightly better result (by $0.3\%$) with comparable computational times. Finally, it is important to note that the ORRT model is highly sensitive to starting points, as shown by both the higher standard deviation and the number of anomalies (in some datasets more than a quarter of the runs)}

\textcolor{blue}{In the comparative analysis with the ORT-L model, the results presented in the final rows of Table \ref{tab:depth3} show that the MRRT $l_2$ model achieves a higher $R^2$ (at least by $2\%$ on average) while maintaining lower standard deviation levels, thus less sensitive to the starting points. As to computational times, excluding datasets with a small number of data points or predictor variables (e.g., airfoil, computer, and yacht) where times are comparable, MRRT $l_2$ keeps the computational time always lower. For instance, in the case of auto mpg, computers, elevators, housing, and kin8nm datasets MRRT $l_2$ achieves accuracy levels between $5.4\%$ and $14.1\%$ higher while keeping computational times almost always substantially lower. While for datasets such as airfoil, delta, puma, and yacht ORT-L is slightly better in terms of accuracy than MRRT $l_2$ (between $0.3\%$ and $3.5\%$ more $R^2$) while maintaining comparable computational times excluding the case of puma where the time of ORT-L is two orders of magnitude higher.}

\textcolor{blue}{Table \ref{tab:perc_gap} reports for depths 2 and 3 the percentual gap in terms of accuracy and time between MRRT $l_2$ and ORT-L. The results indicate that MRRT $l_2$ outperforms ORT-L as the preferred alternative. At depth 2 most of the gaps are positive compared for MRRT $l_2$ with a maximum of $27.74\%$, while as far as time is concerned there is up to $99.58\%$ of time saved. Similarly, at depth 3, MRRT $l_2$ maintains a distinct advantage with a maximum gap of approximately $21.86\%$ in terms of $R^2$ and a substantial time reduction of up to $99.52\%$.}

\begin{table}[H]
\caption{Comparison between MRRT $\ell_2$ and ORT-L with depths $D = 2,3$ in terms of percentual gap of accuracy and computational time.}\label{tab:perc_gap}
\centering
\resizebox{0.7\columnwidth}{!}{
\begin{tabular}{lcccc|cccc}
\hline
          & \multicolumn{4}{c|}{D=2}                                                           & \multicolumn{4}{c}{D=3}                                                           \\ \cline{2-9} 
Dataset   & \multicolumn{2}{c}{$R^2$ improvement $\%$} & \multicolumn{2}{c|}{Time saving $\%$} & \multicolumn{2}{c}{$R^2$ improvement $\%$} & \multicolumn{2}{c}{Time saving $\%$} \\ \cline{2-9} 
          & MRRT $l_2$             & ORT-L             & MRRT $l_2$           & ORT-L          & MRRT $l_2$             & ORT-L             & MRRT $l_2$          & ORT-L          \\ \hline
Abalone   & -                      & 0.72              & 87.62                & -              & 3.49                   & -                 & 83.8                & -              \\
Ailerons  & 1.45                   & -                 & 92.77                & -              & 1.21                   & -                 & 83.74               & -              \\
Airfoil   & 0.538                  & -                 & -                    & 59.88          & -                      & 4.34              & -                   & 58.68          \\
Auto mpg  & 3.82                   & -                 & 58.42                & -              & 6.59                   & -                 & 38.62               & -              \\
Compact   &     -                   & 0.1               & 94.44                & -              & -                      & -                 & 93.41               & -              \\
Computer  & 9.92                   & -                 & -                    & 4.52           & 7.42                   & -                 & -                   & 20.6           \\
Cpu small & 0                      & 0                 & 85.43                & -              & -                      & 0.1               & 86.27               & -              \\
Delta     & 0.57                   & -                 & -                    & 27.14          & -                      & 0.42              & -                   & 41.14          \\
Elevators & 7.26                   & -                 & 91.8                 & -              & 8.87                   & -                 & 81.65               & -              \\
Friedman  & 0.9                    & -                 & 54.3                 & -              & 0.32                   & -                 & 77.02               & -              \\
Housing   & 8.18                   & -                 & 93.29                & -              & 11.08                  & -                 & 90.63               & -              \\
Kin8nm    & 27.74                  & -                 & 95.68                & -              & 21.86                  & -                 & 94.64               & -              \\
Lpga2009  & 3.6                    & -                 & 81.59                & -              & 3.91                   & -                 & 69.99               & -              \\
Puma      & -                      & 0.98              & 99.58                & -              & -                      & 2.72              & 99.52               & -              \\
Yacht     & -                      & 1.5               & -                    & 60.96          & -                      & 0.91              & -                   & 48.06          \\ \hline
\end{tabular}
}
\end{table}

Finally, an interesting comparison can be made with classical Hierarchical Mixtures of Experts (HMEs) models, which can be viewed as a soft variation of tree based methods. In HMEs, branch nodes are gating functions that assign weights for the prediction, which is represented as a weighted combination of the experts represented by the leaf nodes. A comparison with HME models on the 15 datasets is reported in Appendix \ref{appendix:MRRT_HME}.

%Concerning the results with depth $D=2$ in Table \ref{tab:depth2}, comparing the two non-linear formulations, it is easy to see how the MRRTs formulation is almost always able to achieve a higher level of accuracy than the ORRT model while maintaining almost always lower calculation times. Furthermore, looking at the average standard deviation and the number of anomalies, one can see how our model is much less sensitive to starting points. For example, in the case of the Housing dataset, while MRRT reaches a level of accuracy of 0.846 with an average of 4.63 sec CPU time, the ORRT model reaches 0.735 in 10.56 seconds. 

%Looking at the comparison with the ORT L model, we see how excluding the Puma and Yacht datasets, where ORT L  exceeds MRRT by no more than 1.1 $\%$. the MRRT model is able to achieve a noticeable improvement in testing $R^2$ and a remarkable speed up in terms of CPU time. For example, in the case of kin8nm dataset MRRT achieves 0.7226 of testing $R^2$ requiring 44.8 seconds while the ORT L reaches 0.5662 with 1349.19 CPUT ime. Looking at average CPU time  while the MRRT model needs on average 43.3 seconds, the ORT-L model requires 2934.22 seconds.

%Regarding the results with depth $D=3$ of Table \ref{tab:depth3}, in general the MRRT model is able to achieve a remarkable improvements in terms of testing $R^2$ with respect to both alternative models while keeping the CPU time low. Indeed, looking at the last row the MRRT model is able to achieve the higher testing $R^2$ on average, that is 0.8608 against the 0.8413 of the ORT L and the 0.6856 of the ORRT while keeping the CPU time low. The MRRT model requires on average 168.36 second versus the 6257.50 seconds of the ORT L and the 1377.77 seconds of the ORRT. 













\iffalse
\begin{table}[]
\centering
\caption{Comparison between MRRT, MRRT $l_2$, ORT-L and ORRT with depth $D = 2$. Anomaly corresponds to solutions with negative out-of-sample $R^2$. The number of negative $R^2$ for MRRT, MRRT $l_2$ and ORT-L is equal to 0.}\label{tab:depth2}
\resizebox{\textwidth}{!}{\begin{tabular}{lccccccccccccc}
\hline
          & \multicolumn{13}{c}{D=2}                                                                                                                                                  \\ \cline{2-14} 
Dataset   & \multicolumn{3}{c}{MRRT}   & \multicolumn{3}{c}{MRRT $l_2$} & \multicolumn{3}{c}{ORT L}    & \multicolumn{4}{c}{ORRT}                                                     \\ \cline{2-14} 
          & $R^2$  & $\sigma$ & Time   & $R^2$    & $\sigma$  & Time    & $R^2$  & $\sigma$ & Time     & $R^2$  & $\sigma$ & \multicolumn{1}{l}{Time} & \multicolumn{1}{l}{Anomalies} \\ \hline
Abalone   & 0.5514 & 0.0218   & 8.59   & 0.554    & 0.0214    & 8.74    & 0.558  & 0.017    & 70.62    & 0.5254 & 0.03317  & 18.17                    & 8                             \\
Ailerons  & 0.833  & 0.006    & 18.99  & 0.8364   & 0.0056    & 18.95   & 0.824  & 0.0113   & 262.16   & 0.7714 & 0.1353   & 427.73                   & 45                            \\
Airfoil   & 0.7617 & 0.0315   & 5.21   & 0.748    & 0.029     & 5.16    & 0.744  & 0.0159   & 2.07     & 0.5164 & 0.0289   & 1.81                     & 4                             \\
Auto mpg  & 0.8528 & 0.02     & 2.48   & 0.8705   & 0.0237    & 2.47    & 0.838  & 0.028    & 5.94     & 0.8115 & 0.0223   & 0.89                     & 17                            \\
Compact   & 0.9793 & 0.0025   & 35.47  & 0.98     & 0.00168   & 37.17   & 0.981  & 0.0034   & 668.37   & 0.692  & 0.131    & 183.2                    & 11                            \\
Computer  & 0.977  & 0.0186   & 1.97   & 0.9643   & 0.0249    & 1.99    & 0.877  & 0.134    & 1.9      & 0.907  & 0.055    & 0.572                    & 10                            \\
Cpu small & 0.9691 & 0.0032   & 33.78  & 0.9694   & 0.0023    & 31.34   & 0.9703 & 0.0024   & 215.09   & 0.72   & 0.04     & 62.65                    & 6                             \\
Delta     & 0.701  & 0.0064   & 10.96  & 0.701    & 0.0063    & 10.4    & 0.6967 & 0.007    & 7.577    & 0.678  & 0.007    & 8.56                     & 4                             \\
Elevators & 0.8716 & 0.005    & 40.69  & 0.8713   & 0.0047    & 39.55   & 0.812  & 0.0058   & 482.6    & 0.813  & 0.006    & 220.37                   & 26                            \\
Friedman  & 0.8949 & 0.0075   & 134.34 & 0.8943   & 0.0085    & 134.46  & 0.886  & 0.0013   & 294.2    & 0.7226 & 0.0018   & 56.28                    & 6                             \\
Housing   & 0.85   & 0.046    & 2.94   & 0.846    & 0.034     & 2.92    & 0.7816 & 0.0517   & 43.49    & 0.699  & 0.104    & 3.8                      & 7                             \\
Kin8nm    & 0.72   & 0.019    & 19.62  & 0.7226   & 0.0228    & 19.02   & 0.5656 & 0.018    & 439.79   & 0.4116 & 0.012    & 10.95                    & 5                             \\
Lpga2009  & 0.7647 & 0.074    & 2.23   & 0.8907   & 0.0258    & 2.23    & 0.86   & 0.031    & 12.11    & 0.8645 & 0.109    & 0.89                     & 4                             \\
Puma      & 0.8151 & 0.0096   & 45.31  & 0.815    & 0.009     & 44.95   & 0.823  & 0.009    & 10592.25 & 0.216  & 0.032    & 53.54                    & 7                             \\
Yacht     & 0.987  & 0.0058   & 2.54   & 0.976    & 0.0077    & 2.49    & 0.991  & 0.0018   & 0.972    & 0.643  & 0.062    & 0.636                    & 11                            \\ \hline
AVG ARIT  & 0.8352 & 0.01846  & 24.34  & 0.8426   & 0.01516   & 24.12   & 0.8139 & 0.0225   & 873.28   & 0.666  & 0.052    & 70.01                    &                               \\ \hline
AVG GEOM  & 0.8267 & 0.012    & 11.6   & 0.8343   & 0.01094   & 11.48   & 0.8036 & 0.0111   & 66.29    & 0.6352 & 0.031    & 13.12                    &                               \\ \hline
\end{tabular}}
\end{table}



\begin{table}[]
\caption{Comparison between MRRT, MRRT $l_2$, ORT-L and ORRT with depth $D = 3$. Anomaly corresponds to solutions with negative out-of-sample $R^2$. The number of negative $R^2$ for MRRT, MRRT $l_2$ and ORT-L is equal to 0.}\label{tab:depth3}
\centering
\resizebox{\textwidth}{!}{\begin{tabular}{lccccccccccccc}
\hline
          & \multicolumn{13}{c}{D=3}                                                                                                                                \\ \cline{2-14} 
Dataset   & \multicolumn{3}{c}{MRRT}   & \multicolumn{3}{c}{MRRT $l_2$} & \multicolumn{3}{c}{ORT L}   & \multicolumn{4}{c}{ORRT}                                    \\ \cline{2-14} 
          & $R^2$  & $\sigma$ & Time   & $R^2$    & $\sigma$  & Time    & $R^2$  & $\sigma$ & Time    & $R^2$  & $\sigma$ & Time    & \multicolumn{1}{l}{Anomalies} \\ \hline
Abalone   & 0.558  & 0.0267   & 24.55  & 0.564    & 0.0216    & 23.97   & 0.545  & 0.019    & 147.98  & 0.5159 & 0.0667   & 107.59  & 20                            \\
Ailerons  & 0.826  & 0.009    & 50.62  & 0.835    & 0.0043    & 50.48   & 0.8255 & 0.012    & 310.49  & 0.7837 & 0.1165   & 2491.85 & 44                            \\
Airfoil   & 0.816  & 0.039    & 11.23  & 0.807    & 0.0214    & 11.35   & 0.842  & 0.013    & 4.69    & 0.5135 & 0.018    & 9.04    & 20                            \\
Auto mpg  & 0.842  & 0.0412   & 6.18   & 0.873    & 0.0217    & 6.15    & 0.819  & 0.0647   & 10.02   & 0.815  & 0.0245   & 6.81    & 7                             \\
Compact   & 0.9791 & 0.0038   & 72.13  & 0.98     & 0.0027    & 72.72   & 0.9805 & 0.0048   & 1103.46 & 0.721  & 0.034    & 905.65  & 5                             \\
Computer  & 0.973  & 0.018    & 4.02   & 0.9546   & 0.0337    & 4.03    & 0.889  & 0.16     & 3.2     & 0.887  & 0.138    & 4.27    & 14                            \\
Cpu small & 0.9693 & 0.0026   & 57.19  & 0.97     & 0.0025    & 58.67   & 0.9713 & 0.0031   & 427.41  & 0.705  & 0.0724   & 323.2   & 3                             \\
Delta     & 0.7042 & 0.0111   & 28.4   & 0.706    & 0.01      & 29.53   & 0.709  & 0.00768  & 17.38   & 0.672  & 0.027    & 52.68   & 4                             \\
Elevators & 0.8862 & 0.0052   & 97.64  & 0.8838   & 0.0057    & 94.66   & 0.812  & 0.0058   & 515.78  & 0.783  & 0.103    & 1476.75 & 21                            \\
Friedman  & 0.937  & 0.0053   & 310.47 & 0.9376   & 0.0028    & 311.76  & 0.9349 & 0.0006   & 1356.56 & 0.7213 & 0.0123   & 455.75  & 13                            \\
Housing   & 0.809  & 0.083    & 7.23   & 0.872    & 0.0448    & 7.35    & 0.7853 & 0.0833   & 78.4    & 0.715  & 0.061    & 19.14   & 10                            \\
Kin8nm    & 0.787  & 0.0188   & 50.18  & 0.786    & 0.019     & 50.73   & 0.6449 & 0.011    & 946.47  & 0.412  & 0.0104   & 45.9    & 9                             \\
Lpga2009  & 0.8    & 0.113    & 4.92   & 0.8772   & 0.025     & 4.96    & 0.844  & 0.04     & 16.53   & 0.8801 & 0.042    & 4.58    & 8                             \\
Puma      & 0.8838 & 0.0091   & 135.93 & 0.8835   & 0.0088    & 136.51  &  0.907  & 0.  &         & 0.215  & 0.032    & 233.07  & 13                            \\
Yacht     & 0.9905 & 0.0049   & 5.18   & 0.9834   & 0.0048    & 5.41    & 0.992  & 0.0011   & 2.81    & 0.645  & 0.056    & 3.57    & 21                            \\ \hline
AVG ARIT  & 0.8507 & 0.026    & 57.72  & 0.8609   & 0.0152    & 57.88   & x      & x        & x       & 0.6656 & 0.0542   & 409.32  & \multicolumn{1}{l}{}          \\ \hline
AVG GEOM  & 0.8428 & 0.0146   & 27.19  & 0.8534   & 0.0105    & 27.38   & x      & x        & x       & 0.6347 & 0.0422   & 75.0    & \multicolumn{1}{l}{}          \\ \hline
\end{tabular}}
\end{table}

\fi





  







\iffalse

\begin{table}[]
\centering
\renewcommand{\arraystretch}{0.7}
\resizebox{0.7\columnwidth}{!}{
\begin{tabular}{lcccc|cccc}
\hline
                            & \multicolumn{4}{c|}{Depth = 2}                           & \multicolumn{4}{c}{Depth = 3}                            \\ \cline{2-9} 
\multicolumn{1}{c}{Dataset} & \multicolumn{2}{c}{$R^2$ improvement $\%$} & \multicolumn{2}{c|}{Time saving $\%$} & \multicolumn{2}{c}{$R^2$ improvement $\%$} & \multicolumn{2}{c}{Time saving $\%$}  \\ \cline{2-9} 
                            & MRRT $l_2$    & ORT L        & MRRT $l_2$  & ORT L       & MRRT $l_2$    & ORT L        & MRRT $l_2$  & ORT L       \\ \hline 
Abalone                     & 0.65   & -            & 87.23 & -           & 2.47   & -            & 70.18 & -           \\
Ailerons                    & 1.05   & -            & 97.09 & -           & 0.81   & -            & 89.2 & -           \\
Airfoil                     & 0.54   & -            & -           & 16.21 & -             & 5.34  & -           & 37.27 \\
Auto mpg                    & 3.77   & -            & 79.11 & -           & 3.93   & -            & 60.29 & -           \\
Compact                     & 0.12   & -            & 96.79 & -           & 0.18    & -            & 93.08 & -           \\
Computer                    & 6.16   & -            & 54.06 & -           & 7.26   & -            & 23.16 & -           \\
Cpu small                   & 0             & 0            & 93.31 & -           & -             & 0.07  & 88.64 & -           \\
Delta                       & 0.46   & -            & 19.38 & -           & 0.64   & -            & -           & 44.83 \\
Elevators                   & 7.28   & -            & 95.56 & -           & 8.84   & -            & 78.58 & -           \\
Friedman                    & 0.94   & -            & 81.73 & -           & 0.28    & -            & 82.64 & -           \\
Housing                     & 10.72   & -            & 96.54 & -           & 7.71   & -            & 40.58 & -           \\
Kin8nm                      & 27.62   & -            & 96.79 & -           & 22.18    & -            & 94.64 & -           \\
Lpga2009                    & 1.31   & -            & 92.9 & -           & 0.19   & -            & 87.1 & -           \\
Puma                        & -             & 0.99  & 99.62 & -           & x             & x            & x           & x           \\
Yacht                       & -             & 1.17  & 14.25 & -           & -             & 0.83  & -           & 13.89 \\ \hline
\end{tabular}
}
\end{table}

\fi

==> sections/fairness.tex <==
\section{Fairness constraints}\label{sec:fairness}

%\textcolor{red}{In the last decades, we have seen an incredible enhancement and a widespread use of ML and statistical models in order to support decision-making under uncertainty. The main reason for the ML model’s explosion lies in the ability to provide higher level of accuracy by means of algorithmic patterns recognition in data.} 

%\textcolor{red}{Despite this increased usage, many ML are used as black box. As a consequence the decisions these algorithms make are often unclear. Building a model for which it is easy to comprehend why certain decisions or predictions have been made can be problematic in some fields if not even crucial. For example in fields where algorithm decisions need to be explainable (e.g. Medicine) or attributable to certain characteristics due to laws or regulations (e.g. Bank insurance, Autonomous car driving), or where accountability is required.}

%Recently the social impact of ML models has been analysed under a more critical eye by experts and policymakers in order to evaluate whether ML models are unbiased and do not implicitly or explicitly discriminate against underrepresented groups. For example, during the Obama administration, a report \cite{podesta2014big} on big data collection and algorithmic reprocessing warned about harmful biases and risks of discrimination against disadvantaged groups. As a result, several statistical formalizations and mathematical formulations must be considered in order to tackle bias from big data and fairness in different ML models. 

%Concerning building optimal decision trees which take into account fairness measures, we can distinguish recent contributions into two different paradigms: the Continuous Optimization approach and the Mixed-Integer Optimization (MIO) approach.



%Thanks to the structure and the flexibility of the randomized decision trees model, it is possible to directly extend them in order to take into account different measures of fairness for regression tasks. This can be carried out by incorporating appropriate constraints ensuring the desired level of fairness without compromising the overall accuracy.

%To do this the idea is to incorporate this information through the definition of appropriate constraints within which the model must achieve a high performance.

In the last decades, the widespread adoption of ML models for decision-making has been driven by their ability to provide accurate results through algorithmic pattern recognition in data.

Despite this increased usage, many ML models are used as black box, leading to lack of transparency and accountability. As a consequence, the use of ML algorithms in socially sensitive decision making has raised concerns about potential implicit hidden discrimination \cite{mehrabi2021survey}. This concern arises when the training dataset itself exhibits bias, such as marginalization of historically discriminated groups \cite{pedreshi2008discrimination}. Moreover, discrimination can occur if the model errors disproportionately affect certain sensitive groups \cite{adler2018auditing} (e.g., higher misclassification rates for Blacks compared to Whites).

As a result, several statistical formalizations and mathematical formulations have recently been proposed in order to introduce fairness measures in different ML models, including decision trees.

The aim of this section is to introduce group fairness measures within soft decision trees, namely guaranteeing the parity between sensitive groups (e.g., ethnicity or gender).

Let us assume $ G \subset I$ be the subset of data points belonging to a sensitive group and $\bar{G}$ its complementary counterpart (i.e, $\bar{G} = I\setminus G $).
This study aims to consider two distinct group fairness objectives: to prevent discrimination between groups with different values of sensitive characteristics (i.e. \textit{predictive parity}) and to maintain high prediction accuracy (\textit{accuracy assurance}).

%The goal is either to avoid discrimination between groups that possess different values of sensitive characteristics (i.e. \textit{predictive parity}) or to maintain a high level of accuracy in prediction (\textit{accuracy assurance}). 

There are several ways to address \textit{predictive parity}. 
One possibility is to impose that the predictions for a group are not too different from the predictions for non-group individuals:
$$ E(\phi_i(\bm{x}_i,\bm{\w},\bm{\beta})|i \in G) = E(\phi_i(\bm{x}_i,\bm{\w},\bm{\beta})|i \in \bar{G}).$$
Another option is to guarantee that predictions of a specific group are not too different from the predictions of the overall dataset:
$$ E(\phi_i(\bm{x}_i,\bm{\w},\bm{\beta})|i \in G) = E(\phi_i(\bm{x}_i,\bm{\w},\bm{\beta})|i \in I).$$

For both possibilities, we introduce appropriate constraints that are able to impose such \textit{predictive parity}. For $\rho \geq 0$ we introduce the following two constraints to the formulation \eqref{eq:formulation1}:
\begin{equation}
\label{eq:predictive_par1}
 {\Bigg |}\frac{\sum\limits_{i\in G}{ \phi(\bm{x}_i,\bm{\w},\bm{\beta})} }{|G|} - \frac{\sum\limits_{i\in \bar{G}}{ \phi(\bm{x}_i,\bm{\w},\bm{\beta})} }{|\bar{G}|} {\Bigg |} \leq \rho,
\end{equation}
and 
\begin{equation}
\label{eq:predictive_par2}
 {\Bigg |}\frac{\sum\limits_{i\in G}{ \phi(\bm{x}_i,\bm{\w},\bm{\beta})} }{|G|} - \frac{\sum\limits_{i\in I}{ \phi(\bm{x}_i,\bm{\w},\bm{\beta})} }{|I|} {\Bigg |} \leq \rho.
\end{equation}

Concerning the \textit{accuracy assurance}, the idea is to ensure some level of predictive accuracy for groups of individuals within the dataset that are more critical (e.g. underrepresented minority, imbalance dataset). To do so, we can impose that errors on predictions for individuals in a sensitive group do not differ greatly either from a given threshold or from errors on predictions for individuals not in that group. 

For both options, the idea is to constrain the model to prediction error levels that do not exceed a threshold, but instead of using the classical MSE we constrain the absolute error between the prediction and the actual response.



%Another possibility is to guarantee certain level of accuracy for data points belonging to a sensitive group, that is an \textit{accuracy assurance}. In some cases there may be groups of individuals within the dataset that are more critical (e.g. because they are an underrepresented minority) that the model may overlook. In these cases it is necessary to ensure some level of predictive accuracy for those groups. 

%This aspect could be very crucial in ML. Indeed, in the past several machine learning models have shown bias caused by the imbalance within the data corpus used to train these models of the number of instances belonging to a sensitive group\footnote{https://www.nytimes.com/2021/09/03/technology/facebook-ai-race-primates.html}.One possibility is to impose that errors on predictions for individuals in a sensitive group do not differ greatly either from a given threshold or from errors on predictions for individuals not in that group. For both possibilities, the goal is to introduce appropriate constraints that are able to impose such measures without undermining performance in terms of computational time. To do so, the idea is to constrain the model to prediction error levels that do not exceed a threshold, but instead of using the classical \textbf{MSE} we constrain the absolute error between the prediction and the actual response.

Given a threshold $\rho$ the two alternative constraints are:

\begin{equation}
\label{eq:accu_ass1}
    \frac{\sum\limits_{i \in G} |y_i - \phi(\bm{x}_i,\bm{\w},\bm{\beta}) |}{|G|} \leq \rho,
\end{equation}
and
\begin{equation}
\label{eq:accu_ass2}
    \frac{\sum\limits_{i \in G} |y_i - \phi(\bm{x}_i,\bm{\w},\bm{\beta}) |}{|G|} \leq \rho \frac{\sum\limits_{i \in \bar{G}} |y_i - \phi(\bm{x}_i,\bm{\w},\bm{\beta}) |}{|\bar{G}|}.
\end{equation}
It is important to note that both constraints are linear and this has a minor impact on computational time while keeping them very low. Furthermore, in formulation \ref{eq:formulation1}, which is solved with the decomposition algorithm, both \textit{predictive parity} and \textit{accuracy assurance} constraints are naturally introduced in the leaf node step (\textbf{LN Step}). This results in a transition for the \textbf{LN Step} to a convex quadratic programming problem that, unlike other types of formulations where the introduction of fairness results in a significant level of complexity (see e.g. \cite{blanquero2021sparse}), can be solved by efficient algorithms.


Concerning \textit{predictive parity}, we apply the two constraints \eqref{eq:predictive_par2} and \eqref{eq:predictive_par1} on three well-known different datasets to assess fairness capabilities: Housing, MEPS (Healthcare expenditures of individuals) and LSAC (National Longitudinal Study Bar Passage). 
The datasets and experimental setting details can be found in Appendix \ref{appendix:MRRT_HME}.

The Figure \ref{fig:predictive} shows the results in terms of training predictive parity, testing predictive parity and testing $R^2$ of the two \textit{predictive parity} measures for the three datasets. In particular, the x-axis represents the value of $\rho$, the left y-axis the predictive parity level while the right y-axis describes the testing $R^2$. For each $\rho$ value, testing $R^2$ is denoted by an orange circle, while training and testing predictive parity levels are represented by the blue and green bars, respectively. The horizontal line represents the testing $R^2$ as $\rho$ decreases. The left column shows results with the \eqref{eq:predictive_par1} constraint, and the right column shows the ones with the \eqref{eq:predictive_par2} constraint. The MRRT without any constraint is given by the value $\rho=$ inf.


Concerning Housing dataset, we see that for both tasks the constraints positively affect both training and testing phases keeping the prediction levels high (i.e. testing $R^2$ does not seem to suffer much). As to LSAC dataset, we see a considerable impact on prediction parity in both training and testing phases at the cost of reducing testing predictive capabilities. For the MEPS dataset, the constraints have a huge impact at the cost of reducing the testing $R^2$ as $\rho$ decreases.

\begin{table}[]
\centering

\caption{Results for the  \textit{accuracy assurance} constraint \eqref{eq:accu_ass1} on Auto-mpg dataset.}
\label{tab:tabfair}
\resizebox{0.7\columnwidth}{!}{
\iffalse
\begin{tabular}{clcclcclcclc}

\hline
\multicolumn{1}{l}{}       &  & \multicolumn{10}{c}{Boston Housing}                                                                                                                                                                      \\ \hline
\multicolumn{1}{l}{$\rho$} &  & \multicolumn{2}{c}{$accuracy\, assurance$} &  & \multicolumn{2}{c}{$R^2$ over \footnotesize{$G$}} &  & \multicolumn{2}{c}{$R^2$ over \footnotesize{$\bar{G}$}} &  & testing $R^2$  \\ \hline
                           &  & train                 & test               &  & train                           & test                           &  & train                              & test                              &  &        \\ \hline
$\infty$                   &  & 2.08036               & 2.514              &  & 0.8456                          & 0.7771                         &  & 0.8917                             & 0.772                             &  & 0.7934 \\
2                          &  & 1.93833               & 2.511              &  & 0.85477                         & 0.7677                         &  & 0.8551                             & 0.7566                            &  & 0.786  \\
1.75                       &  & 1.74385               & 2.473              &  & 0.8639                          & 0.7412                         &  & 0.8045                             & 0.698                             &  & 0.757  \\ \hline
\end{tabular}

%\newline
\vspace*{20pt}
%\newline
\fi
\begin{tabular}{clcccccccccc}
\hline
\multicolumn{1}{l}{}       &  & \multicolumn{10}{c}{Auto-mpg}                                                                                                                                                                                                         \\ \hline
\multicolumn{1}{l}{$\rho$} &  & \multicolumn{2}{c}{$accuracy\, assurance$} & \multicolumn{1}{l}{} & \multicolumn{2}{c}{$R^2$ over \footnotesize{$G$}} & \multicolumn{1}{l}{} & \multicolumn{2}{c}{$R^2$ over \footnotesize{$\bar{G}$}} & \multicolumn{1}{l}{} &  $R^2$ over $I$   \\ \hline
                           &  & train                & test                & \multicolumn{1}{l}{} & train                  & test                    & \multicolumn{1}{l}{} & train                      & test                      & \multicolumn{1}{l}{} &   test      \\ \hline
-                   &  & 0.0918               & 0.10325             &                      & 0.3253                 & 0.0441                  &                      & 0.9022                     & 0.861                     &                      & 0.85868 \\
0.085                      &  & 0.08248              & 0.0999              &                      & 0.4419                 & 0.16483                 &                      & 0.89657                    & 0.8532                    &                      & 0.855   \\
0.08                       &  & 0.0784               & 0.0998              &                      & 0.4747                 & 0.2521                  &                      & 0.8976                     & 0.8438                    &                      & 0.8473  \\ \hline
\end{tabular}
}
\end{table}






For the \textit{accuracy assurance} we apply the constraint \eqref{eq:accu_ass1} on Auto-mpg dataset. Since the dataset do not have any sensitive group we artificially created it. For more detailed information, please refer to Appendix \ref{}. 

%The Figure \ref{fig:accuracyassurance} shows the results of the \textit{accuracy assurance} measures for Auto-mpg. The MRRT without any restriction is given by the value $\rho=$ -. 



Table \ref{tab:tabfair} reports the results in terms of training \textit{accuracy assurance}, testing \textit{accuracy assurance} and testing $R^2$ for Auto-mpg dataset. We also include training and testing $R^2$ on the subsets of $I$ identified by $G$ and $\bar{G}$. It is easy to see that the constraint affect both the training and testing phase without a significant impact on the testing $R^2$. An interesting aspect is to see how the prediction level $R^2$ on the group $G$ increases as $\rho$ decreases in both training and testing, and this is at the expense of the complementary group $\bar{G}$. This shows how the constraint is able to give more weight in terms of prediction to the group $G$.

\begin{figure}[h]

   \begin{minipage}{0.5\textwidth}
     \centering
     \textbf{Between groups}\par\medskip
     \includegraphics[width=1.125\linewidth]{images/housing0.png}
   \end{minipage}
   \hfill
   \begin{minipage}{0.5\textwidth}
     \centering
     \textbf{Overall}\par\medskip
     \includegraphics[width=1.125\linewidth]{images/housing-1.png}

   \end{minipage}
   
   \begin{minipage}{0.5\textwidth}
     \centering
     
     \includegraphics[width=1.125\linewidth]{images/lsac0.png}
   \end{minipage}
   \hfill
   \begin{minipage}{0.5\textwidth}
     \centering
     
     \includegraphics[width=1.125\linewidth]{images/lsac-1.png}

   \end{minipage}
   
   \begin{minipage}{0.5\textwidth}
     \centering
     
     \includegraphics[width=1.125\linewidth]{images/meps0.png}
   \end{minipage}
   \hfill
   \begin{minipage}{0.5\textwidth}
     \centering
     
     \includegraphics[width=1.125\linewidth]{images/meps-1.png}

   \end{minipage}
   \caption[]{Results of MRRT model with \textit{predictive parity} constraints. The blue bar represents the results on the training set while the green one the results on the test set. The orange line is the testing $R^2$.}
   \label{fig:predictive}
\end{figure}



==> sections/implementation_new_old.tex <==
\section{Practical implementation}\label{subsec:implementation}
In this section, we present the implemented NOME decomposition algorithm, which, alternating the nonconvex optimization of branching node variables (\textbf{BN Step}) and the convex optimization of leaf node variables (\textbf{LN Step}), results to be a version of the NDGS general algorithm described in Section \ref{subsec:scheme}.

The NOME algorithm is an asymptotically convergent decomposition method, which embeds in the first steps two heuristic procedures: a clustering-based initialization, and a samples reassignment procedure. The use of such heuristics help to mitigate instability issues due to the high complexity of the objective function, e.g., early convergence to poor solutions and degenerate routing of almost all samples towards a single path in the tree. \textcolor{red}{Indeed, in addition to the problems of least squares associated to each leaf nodes, the problem of routing and assigning data points to branch nodes pose significant computational challenges for generic solvers.} 

The remainder of this section is organized as follows. In Section \ref{subsec:algorithm} algorithm NOME is described in detail together with all convergence aspects, Section \ref{subsec:reass} is devoted to the description of the reassignment heuristic, while Section \ref{subsec:init} describes the initialization strategy, Section \ref{sec:preliminary_ex} presents some preliminary results showing the various contributions of the algorithm components together with the initialization procedure.

%In this section we present the implemented decomposition algorithm, the so-called NOME, which is a version of the NDGS general algorithm presented in Section \ref{subsec:scheme}. Indeed, NOME alternates a nonconvex optimization with respect to the branching node variables (\textbf{BN Step}), with a convex optimization with respect to a subset of leaf node variables (\textbf{LN Step}).

%Although being asymptotically convergent according to theory presented in Section \ref{subsec:convergence}, NOME embeds in the first steps two heuristic procedures: a clustering-based initialization, and a samples reassignment procedure. Such heuristics are helpful in reducing instability phenomena, in particular early convergence to poor solutions and degenerate routing of almost all samples towards a single path in the tree,  which often affect the training of (randomized) regression trees. \textcolor{red}{The main reason for these poor solutions is the high complexity of the objective function. Indeed, in addition to the problems of least squares associated to each leaf nodes, the problem of routing and assigning instances in the branching nodes turns out to be highly difficult to handle with a generic solver. The previous drawbacks favour the occurrence of failures in which negative $R^2$ are obtained, referred here as ``\textit{anomalies}"}. 




\subsection{The algorithm description}\label{subsec:algorithm}
Before presenting the details of algorithm NOME, it is necessary to comment on a crucial aspect concerning the nonconvex \textbf{BN Step}. To prevent oscillating behaviour of the decomposition method and to ensure asymptotic convergence it is important to satisfy \textsc{Condition} \ref{con:2} (reported in Section \ref{subsec:convergence}) in the \textbf{BN Step} update. This can be easily obtained by using the partial steepest descent direction in tandem with the well-known Armijo method (see e.g., \cite{Bertsekas/99}). That is, given $W^k_B$, then $\bm{\w}_{W^k_B}^{k+1}$ is set equal to the following Armijo update

\begin{equation}
\label{eq:steepest}
  \bm{\w}_{W^k_B}^{k} + \alpha^k_{W^k_B} \bm{d}_{W^k_B}^k,
\end{equation}


\noindent where $\bm{d}_{W^k_B}^k = - \nabla_{\bm{\w}_{W^k_B}}E(\bm{\w}^k,\bm{\beta}^k)$, and the step length $\alpha^k_{W^k_B}$ is computed through Algorithm \ref{alg:Armijo} reported below, starting from an initial guess $a > 0$.

\begin{algorithm}[H]
\caption{Armijo method}
\label{alg:Armijo}
$\bm{Input}: a\,>\,0;\, \gamma\, \in\, (0,1);\, \delta\,\in\,(0,1);\,(\bm{\w},\bm{\beta});\,J\\$ 
$\bm{Output}:\alpha_J.$
{\fontsize{10}{12}\selectfont
\begin{algorithmic}[1]
\Procedure{ArmijoMethod}{$a,\gamma,\delta,(\bm{\w},\bm{\beta}),J$}
\State $\alpha \gets a$
\While{$ E(\bm{\w}_{J} + \alpha \bm{d}_{J},\bm{\w}_{\bar J},\bm{\beta}) < E(\bm{\w},\bm{\beta}) -\gamma \alpha \|\nabla_{J}E(\bm{\w},\bm{\beta}) \|^2 $}
\State $\alpha \gets \delta \alpha$

\EndWhile
\State $\alpha_J \gets \alpha$
\State \textbf{return} $\alpha_J$
\EndProcedure
\end{algorithmic}
}
\end{algorithm}


%By adapting the result proved in \cite{grippo2015decomposition} to our MRRT framework, it is possible to state some theoretical properties of Algorithm \ref{alg:Armijo} needed for the asymptotic convergence of Algorithm NOME (stated in Proposition \ref{prop:prop3}) and reported in the next proposition, whose proof can be found in Appendix.

As detailed in the Electronic Companion \ref{subsec:ec-1-armjio}, it is possible to show that the adaptation of the Armjio method to the MRRT framework (as reported in Algorithm \ref{alg:Armijo}), inherits some theoretical properties proved in \cite{grippo2015decomposition} in a different context, which are useful from both a practical and an asymptotic convergence point of view. Indeed, at the \textbf{BN Step}, the Armijo update acts as a reference point if a different method is used to determine $\bm{\w}_{W^k_B}^{k+1}$. Let us denote the Armijo update computed as in \eqref{eq:steepest} as $\bm{\w}^{ref}_{W^{k}_B}$, and the alternative candidate point as $\hat{\bm{\w}}_{W^k_B}$. If we set $\bm{\w}_{W^k_B}^{k+1}=\hat{\bm{\w}}_{W^k_B}$, then convergence is ensured provided the following two conditions are satisfied  
\begin{equation}
\label{eq:descreasing1}
    E(\hat{\bm{\w}}_{W^k_B}^k,\bm{\w}_{\bar W^k_B}^k,\bm{\beta}^k) \leq E(\bm{\w}^{ref}_{W^{k}_B},\bm{\w}_{\bar W^k_B}^{k},\bm{\beta}^k),
\end{equation}
and
\begin{equation}
\label{eq:decreasing2}
    E(\hat{\bm{\w}}_{W^k_B}^k,\bm{\w}_{\bar W^k_B}^k,\bm{\beta}^k) \leq E(\bm{\w}^k,\bm{\beta}^k) - \tau \|\hat{\bm{\w}}_{W^k_B}^k - \bm{\w}_{W^k_B}^k \|^2,
\end{equation}
for a given $\tau > 0$. Condition \eqref{eq:decreasing2} is necessary to guarantee that the convergence of the function values implies $\| \bm{\w}_{W^k_B}^{k+1} - \bm{\w}_{W^k_B}^{k}\| \to 0$, which for the Armijo point $\bm{\w}^{ref}_{W^k_B}$ is automatically enforced by $(ii)- a)$ in Proposition \ref{prop:prop2} proved in the Electronic Companion \ref{subsec:ec-1-armjio}.\par 
Now, we are ready to present the decomposition method NOME, whose scheme is reported in Algorithm \ref{alg:Decomposition1}. After initializing the starting solution $(\bm{\w^0},\bm{\beta^0})$ via the $\textsc{InitializationStrategy}$ procedure (described below in Section \ref{subsec:init}), the algorithm is structured as a main external loop of macro iterations, indicated by variable $it$ and iterated until a generic termination test is verified. At each macro iteration $it$, an internal loop of inner iterations $k$ iteratively selects a branching node $t\in \tau_B$ at a time to construct the working set. In particular, $t$ and the set of indices of its branching node descendants (denoted as ${\cal C}_B(t)$) are inserted in $W_B$. Similarly, $W_L$ is defined as the set of all indices of leaf nodes which are descendant of $t$ (denoted as ${\cal C}_L(t)$). The only exception is when $t$ is the root node and $D > 1$. In this case $W_B \equiv \{t\}$ and $W_L \equiv \emptyset$. Once determined $W_B$ and $W_L$, \textbf{BN Step} and \textbf{LN Step} are sequentially performed.

Regarding the $\textbf{BN Step}$, the branching node variables subvector $\bm{\w}_{W^k_B}$ is actually updated only if the norm of the partial gradient $\| \nabla_{{W^k_B}}E(\bm{\w}^k,\bm{\beta}^k)\|$ is greater than a certain decreasing threshold $\theta_{\w}^k$. In such a case, a reference update subvector $\bm{\w}_{W^k_B}^{ref}$ is computed by means of % a s a step $\alpha_{W^k_B}^k$ along the partial antigradient direction $\nabla_{W^k_B}E(\bm{\w}^k,\bm{\beta}^{k})$, where $\alpha_{W^k_B}^k$ is determined by a standard Armjio linesearch step (see e.g., Bertsekas \cite{Bertsekas/99}) through the \textsc{ArmijoMethod} procedure.
the Armijo linesearch described above.
%As detailed in Section \ref{subsec:pract-theo}, the Armijo reference point is used both as a practical guide to prevents oscillation during the iteration progress, and to ensure theoretical asymptotic convergence. 
Then, %for $k \leq Q$ (where $Q$ is a positive integer set by the user),
the \textsc{UpdateBranchNode} procedure (described in detail in Section \ref{subsec:reass}) computes a new candidate point $\hat{\bm{\w}}_{W^k_B}$ either by any standard unconstrained minimization algorithm, or by a specific heuristic method allowing to induce balancing of data distribution within the branching nodes whenever data are particularly imbalanced. The data imbalance tolerance is handled by the thresholds $\bm{\epsilon}_1, \bm{\epsilon}_2 \,\text{and}\, \bm{\epsilon}_3$.  %This second possibility is considered when certain conditions related to the balancing of the instances within the block are met. 
The heuristic method is helpful to improve stability during the initial stages of the algorithm. At the same time to ensure convergence for sufficiently large $k$ (i.e., $k > Q$ where $Q$ is a positive integer set by the user) the new point will be taken only if it satisfies conditions \eqref{eq:descreasing1} and \eqref{eq:decreasing2}, otherwise Armijo reference update is taken (see Steps 17-20).

Also the \textbf{LN Step} is actually performed only if the norm of the partial gradient $\| \nabla_{{W^k_L}}E(\bm{\w}^{k+1},\bm{\beta}^k) \|$ is greater than $\theta_{\beta}^k$. The optimization of the leaf node variables subvector $\bm{\beta}_{W^k_L}^{k}$ corresponds to a linear least-squares problem thus we can minimize it either through an iterative method for convex quadratic function or by a direct method for the linear least-squares problem.

%\textcolor{blue}{Notice that for both \textbf{BN Step} and \textbf{LN Step}, whenever $k \leq Q$, no specific restrictions are imposed for the updates $\bm{\w}_{W^k_B}^{k+1}, \bm{\beta}_{W^k_L}^{k+1}$. Among many possible choices, this methodological freedom allows to take into account only a subset of data points in the resolution of each subproblem so as to speed up the first iterations. In particular, in our implementation, for a given current node $t$ we consider only data points falling into $t$ with a probability larger than 0.5 in the optimization problems related to the \textbf{BN Step} and \textbf{LN Step}, as these points are considered more ``relevant" when determining variables involved in sets $W_B^k$ and $W_L^k$ induced by $t$. Notice that this specific choice should be not confused with a mini-batch sample-based decomposition approach (see e.g.,[]), as the number of samples falling into a node with a certain probability cannot be controlled a priori.}

\textcolor{red}{Notice that for both \textbf{BN Step} and \textbf{LN Step}, whenever $k \leq Q$, no specific restrictions are imposed for the updates $\bm{\w}_{W^k_B}^{k+1}, \bm{\beta}_{W^k_L}^{k+1}$. Among many possible choices, this methodological freedom allows to consider a proxy of the subproblem and/or to take into account only a subset of data points in the resolution of each subproblem so as to speed up the first iterations.} 

\textcolor{red}{In particular, in our specific implementation we employ two strategies to enhance the efficiency and speed of the \textbf{BN Step} and \textbf{LN Step} in the subproblem. First, for a given current node $t$, the objective function related to the associated subproblem does not take into account the probabilities for data points $i$ to fall into node $t$. In simpler terms, during the optimization of the \textbf{BN Step} and \textbf{LN Step}, node $t$ is treated as if it were the root node of the subtree related to the subproblem. Second, in the optimization problems of  \textbf{BN Step} and \textbf{LN Step} related to current node $t$ we consider only the data points falling into $t$ following the branches with highest probability. This approach allows us to focus on those data points that are considered more "relevant" when determining variables involved in sets $W_B^k$ and $W_L^k$ induced by $t$. Notice that this specific choice should not be confused with a mini-batch sample-based decomposition approach, as the number of data points falling into a node with a certain probability cannot be controlled a priori.}\par 
At the end of each inner iteration the parameters $\bm{\epsilon}_1, \bm{\epsilon}_2 \,\text{and}\, \bm{\epsilon}_3$ controlling the data imbalance are decreased. As it will be specified in the \textsc{UpdateBranchNode} scheme, the smaller are these parameters the more data imbalance is allowed. 

\begin{algorithm}[h]
\caption{Decomposition algorithm}
\label{alg:Decomposition1}
$\bm{Input}: depth \,\bm{D}; training\,data \, \bm{X},\bm{y};\,max\,iterations\,\bm{Max\_iter}; \bm{\epsilon_{1}}^0,\,\bm{\epsilon_{2}}^0,\,\bm{\epsilon_{3}}^0,\,\bm{\zeta},\,\theta_{\w},\, \theta_{\beta} \in [0,1)\,$ 
%\vspace{-5pt}
$\\ with\, \bm{\epsilon_{1}}\, >\,\bm{\epsilon_{2}};\,\upsilon \in [0,1);\, Q \in \mathbb{N}, \tau>0.$ 
%\vspace{-10pt}
$\\ \bm{Output}:\,optimal\, values\, \bm{\w^{*}},\,\bm{\beta^{*}}.$
\vspace{-10pt}
  {\fontsize{10}{12}\selectfont
  \begin{algorithmic}[1]
  \Statex {} 
    \State $(\bm{\w}^{0},\bm{\beta}^{0}) \gets\textsc{InitializationStrategy}(\bm{D},\bm{v},\bm{X})$
    \Procedure{Decomposition}{$\bm{D},\bm{X},\bm{y},\bm{\w^0},\bm{\beta^0},\bm{\epsilon_{1}},\bm{\epsilon_{2}},\bm{\epsilon_{3}},\bm{\gamma},\theta_{\w},\theta_{\beta},\upsilon$}
      
      \State $\bullet$ $(\bm{\w}^{*},\bm{\beta}^{*}) \gets \bm{\w}^{0},\bm{\beta}^{0}$
      \State $\bullet$ $\bm{\epsilon_{1}},\,\bm{\epsilon_{2}},\,\bm{\epsilon_{3}}\gets \bm{\epsilon_{1}}^0,\,\bm{\epsilon_{2}}^0,\,\bm{\epsilon_{3}}^0$
      \State $\bullet$ $error_{best} \gets E(\bm{\w}^{*},\bm{\beta}^{*})$
      \State $\bullet$ $k \gets 0,\, it \gets 1,$
      \While{$ it < \bm{Max\_iter}\,and\,$ not {\it termination test}}
       
        \For{$ t = 1,...,|\tau_B| $}\Comment{loop over the branching nodes}
        
        \If{$t == 1\,\text{and}\, \bm{D} > 1$}
        \State $W^k_B \gets \{t\}, \, W^k_L \gets \emptyset$
        \Else
        \State $W^k_B \gets \{t,{\cal C}_{B}(t)\}, \, W^k_L \gets {\cal C}_{L}(t)$
        \EndIf
        
        %\State $W^k_B \gets \{t\}, \, W^k_L \gets children_leaf(t)$
       \Statex
        \Statex  {$\triangleright$ \, \textbf{BN Step}} \textit{(Optimization of branching nodes parameters)}
        
        \If{$\| \nabla_{{W^k_B}}E(\bm{\w}^k,\bm{\beta}^k) \| \leq (\theta_{\w})^k$}
        \State $\bm{\w}^{k+1}\gets \bm{\w}^{k}$
        \Else
        \State $\bullet$ $\alpha_{W^k_B}^k \gets \textsc{ArmijoMethod}(a,\gamma,\delta,(\bm{\w}^{k},\bm{\beta}^k),W^k_B)$
        \State $\bullet$ $\bm{\w}_{W^k_B}^{ref} \gets \bm{\w}_{W^k_B} - \alpha_{W^k_B}^k \nabla_{W^k_B}E(\bm{\w}^k,\bm{\beta}^{k})$
        \State $\bullet$ $\hat{\bm{\w}}_{W^k_B} \gets $\textsc{UpdateBranchNode}$(t,W^k_B,\bm{\w}^{k}_{W^k_B},\bm{X},\bm{\epsilon_{1}},\bm{\epsilon_{2}},\bm{\epsilon_{3}})$ %\Comment{technique that   satisfies }
        
        
            
            
        \If{($\hat{\bm{\w}}_{W^k_B}$ satisfies \eqref{eq:descreasing1}- \eqref{eq:decreasing2}) or ($k \leq Q $)} 
            \State $\bm{\w}_{W^k_B}^{k+1} \gets \hat{\bm{\w}}_{W^k_B}$
        \Else
            \State $\bm{\w}_{W^k_B}^{k+1} \gets \bm{\w}_{W^k_B}^{ref}$
        \EndIf
        
        
        
        
        
        \EndIf
        
        
        \Statex
        \Statex  {$\triangleright$ \, \textbf{LN Step}} \textit{(Optimization of leaf nodes parameters)}
        
        \If{$\| \nabla_{{W^k_L}}E(\bm{\w}^{k+1},\bm{\beta}^k) \| \leq (\theta_{\beta})^k$}
        \State $\bm{\beta}^{k+1}\gets \bm{\beta}^{k}$
        \Else
        \textcolor{blue}{\If{$k \leq Q $} 
            \State compute $\bm{\beta}_{W^k_L}^{k+1} $ by any method
        \Else
            \State compute $\bm{\beta}_{W^k_L}^{k+1}$ such that \\ \qquad \qquad \qquad \;\;\;\, $E(\bm{\w}^{k+1},\bm{\beta}^{k+1})\leq E(\bm{\w}^{k+1},\bm{\beta}^{k})\; \textbf{and} \; \| \nabla_{W^k_L}E(\bm{\w}^{k+1},\bm{\beta}^{k+1}) \| \leq (\upsilon)^k$
        \EndIf
        }
        
        %\State compute $\bm{\beta}_{W^k_L}^{k+1}$ such that $E(\bm{\w}^{k+1},\bm{\beta}^{k+1}) \leq E(\bm{\w}^{k+1},\bm{\beta}^{k})\; \textbf{and}\; \| \nabla_{W^k_B}E(\bm{\w}^{k+1},\bm{\beta}^{k+1}) \| \leq (\upsilon)^k$ \Statex
        
        \EndIf
        \If{$E(\bm{\w}^{k+1},\bm{\beta}^{k+1})< error_{best}$}
        \State $\bullet$ $error_{best} \gets E(\bm{\w}^{k+1},\bm{\beta}^{k+1})$
        \State $\bullet$ ($\bm{\w}^{*},\bm{\beta}^{*}) \gets (\bm{\w}^{k+1},\bm{\beta}^{k+1})$
        \EndIf
        %\State \texttt{left_{t} = descendant(t,right=\bm{True})}
        \State $k \gets k + 1$
        \EndFor
	  \State $\bullet$ $\bm{\epsilon_{1}},\,\bm{\epsilon_{2}},\,\bm{\epsilon_{3}} \gets \bm{\zeta}\cdot\bm{\epsilon_{1}},\,\bm{\zeta}\cdot\bm{\epsilon_{2}},\,\bm{\zeta}\cdot\bm{\epsilon_{3}}$
	  \State $\bullet$ $it \gets it + 1$
      \EndWhile\label{Decompositiondwhile}
      \State \textbf{return} $(\bm{\w}^{*},\bm{\beta}^{*})$
    \EndProcedure
  \end{algorithmic}
  }
\end{algorithm} 
 



%Thanks to \textbf{Proposition} \ref{prop:prop2} assuming that at each step of the subsequence we apply steepest direction in tandem with Armijo's step length as in \eqref{eq:steepest}, since the stepsize is bounded above, the convergence of the function values implies that the subsequence satisfies $\|\bm{\w}_{W^k_B}^{k+1} - \bm{\w}_{W^k_B}^{k} \| \rightarrow 0$ as $k \to \infty$. 

 

It is important to note that, to preserve asymptotic convergence, it is sufficient to impose conditions \eqref{eq:descreasing1} and \eqref{eq:decreasing2} on $\hat{\bm{\w}}_{W^k_B}^k$ only for sufficiently large $k$.
%After the \textbf{BN Step} phase we obtain a point $(\bm{\w}^{k+1},\bm{\beta}^k)$.


In Proposition \ref{prop:prop3} (proved in the Electronic Companion \ref{subsec:ec-1-conv-dec}) we establish the convergence properties of NOME, assuming that it generates an infinite sequence $\{(\bm{\w}^k,\bm{\beta}^k)\}$ of points.
\begin{proposition}
\label{prop:prop3}
Given an infinite sequence $\{(\bm{\w}^k,\bm{\beta}^k)\}$ generated by Algorithm NOME. The following holds:
\begin{enumerate}[label={\arabic*)}]
    \item $\{(\bm{\w}^k,\bm{\beta}^k)\}$ has a limit points.
    \item The sequence $\{E(\bm{\w}^k,\bm{\beta}^k)\}$ converges to a limit.
    \item We have $\lim\limits_{k \to \infty}\|\bm{\beta}^{k+1} -\bm{\beta}^k\|=0 $
    \item For any $ t \in \tau_B$, we have $$\lim\limits_{k \to \infty}\| \bm{\w}_{t}^{k+1} - \bm{\w}_{t}^{k} \|=0$$
    \item Every limit point of $\{(\bm{\w}^k,\bm{\beta}^k)\}$ is a stationary point of $E(\bm\w,
\bm\beta)$ in \eqref{eq:obj}.
\end{enumerate}
\qedblack
\end{proposition}

\subsection{Optimization strategies in the BN Step}\label{subsec:reass}

\textcolor{blue}{During the \textbf{BN Step} of Algorithm \ref{alg:Decomposition1} the new point can be calculated by means of the \textsc{UpdateBranchNode} procedure, as outlined in Algorithm \ref{alg:updatebranching}. \textsc{UpdateBranchNode} considers two scenarios based on how the ancestor node $t$ of $W_B^k$ addresses data points towards its two children nodes: either the distribution of data points is sufficiently uniform, or it is highly imbalanced.}

\textcolor{blue}{To this aim, we consider the set of data points falling into the node $t$ and denoted as $I_t$, the one obtained by setting an appropriate threshold on the sigmoid functions in the ancestors node of $t$, simulating a deterministic behaviour as done in prediction phase (see \eqref{eq:prediction_model}). We also define the two children nodes of $t$ as $left_t$ and $right_t$, and the subsets of data points in these nodes as $I_{left_t}$ and $I_{right_t}$, respectively.}


In the first scenario, data points are sufficiently balanced, i.e. for a given threshold $\bm{\epsilon_{1}} \in (0,1)$ $\bm{\epsilon_{1}} < \frac{|I_{left_{t}}|}{|I_{t}|} < 1 - \bm{\epsilon_{1}}$. Then, the new candidate point is obtained through any nonlinear unconstrained minimization algorithm (e.g., a Newton, a Quasi-Newton or a conjugate gradient method).

In the second scenario, where $\frac{|I_{left_{t}}|}{|I_{t}|} \leq \bm{\epsilon_{1}}$ or\, $\frac{|I_{left_{t}}|}{|I_{t}|} \geq 1 - \bm{\epsilon_{1}}$, only the variables associated to ancestor $t$ are actually optimized as the aim is solely to improve the balance of data points passing through it. The candidate point is obtained by taking into account the level of imbalance. In particular, if for a given threshold $\bm{\epsilon_{2}} < \bm{\epsilon_{1}}$ we have $\bm{\epsilon_{2}} < \frac{|I_{left_{t}}|}{|I_{t}|} < 1 - \bm{\epsilon_{2}}$, the imbalance is moderate and the variables associated to $t$ are obtained by optimizing (through any unconstrained optimization method as in the first scenario) a proxy of the original objective function based on a Balanced Logistic Regression (BLR) function which tends to improve the balance of data points routed in $t$.
The BLR objective function is as follows:
\begin{equation}
\label{eq:reshuffle}
 -\frac{1}{|I_t|} \sum_{i \in I_t} w_ic_iln(p_{it}(\bm{x}_i)) + w_i(1 - c_i)ln(1-p_{it}(\bm{x}_i))  
\end{equation}


\noindent where $c_i = 0$ and $w_i = \frac{|I_t|}{2|I_{left_t}|}$ if the data point $i\in I_{left_t}$, $c_i = 1$ and $w_i = \frac{|I_t|}{2|I_{right_t}|}$ otherwise.


If $\frac{|I_{left_{t}}|}{|I_{t}|} \leq \bm{\epsilon_{2}}$ or\, $\frac{|I_{left_{t}}|}{|I_{t}|} \geq 1 - \bm{\epsilon_{2}}$, the imbalance is considered strong. Then, the optimization of the BLR function is combined with a prior reassignment heuristic used to force data points balance. The heuristic works by moving a fraction $\bm{\epsilon}_3 \in (0,1)$ of data points from the children node with the largest number of them to the other children node. The reassigned data points are those corresponding to larger error values in the partial objective function related to the subtree with the first ancestor $t$, which are considered the more likely to be addressed in the wrong children node. Formally, for a given data point $i$ its partial error is computed as follows:
\begin{equation}
   \label{eq:partial_objective}
    \sum_{t\in {\cal C }_L(t)}P_{it}(\bm{\w})\cdot(\hat y_{it}(\bm{\beta}_t)-y_{i})^{2}.
\end{equation}
The choice of data points to be moved can be also randomized, but preliminary experiment showed that the residual based selection is more effective.

%Whenever the distribution of data among branching nodes is too imbalanced, the idea is to perturb the data points distribution with a reassignment heuristic. The reassignment heuristic is a procedure to both route the data points in the right subproblem and to balance the distribution of data points among the branching nodes of the subtree. This ensures greater stability in the training phase by directing optimization towards solutions that would otherwise be difficult to achieve.

%Concerning the number of data points involved in each subproblem the proposed algorithm considers only data points that falls into the branching node related to the subproblem. It is possible to establish the instances which fall into the subtree, setting an appropriate threshold on the logistic function in the ancestor node of branching node.

%We need to introduce $\bm{\epsilon}_1$ and $\bm{\epsilon}_2$ which represent different thresholds for the assignment of data points in order to manage the possible data imbalance.
%For each branching node $t$ we identify the indices of the children nodes $I_{left_t}$ and $I_{right_t}$. 
%If the imbalance between the data of the child nodes does not exceed the threshold $\epsilon_1$ we optimize the variables through a convergent technique, otherwise we check if the imbalance is greater than the second threshold $\epsilon_2$.
%If the imbalance between the data of the child nodes does not exceed the threshold $\epsilon_1$ we optimize the subproblem with respect $\bm{\w}_{W^k_B}$ through a unconstrained convergent nonlinear optimization algorithm, otherwise we check if the imbalance is greater than the second threshold $\epsilon_2$. If the imbalance is higher than the threshold $\epsilon_2$ we apply the procedure \textit{BalancedLogisticRegression} with reshuffling, otherwise the procedure \textit{BalancedLogisticRegression} is applied without reshuffling.

It is important to emphasize that in the case where the BLR function is used, it is very unlikely that the two acceptance conditions \eqref{eq:descreasing1}- \eqref{eq:decreasing2} in Algorithm \ref{alg:Decomposition1} will be satisfied, as the problem to be solved is a proxy of the original one. Nonetheless, a periodical optimization of the BLR function provides a very effective stabilization of Algorithm \ref{alg:Decomposition1} during the first macro iterations, avoiding to get stuck in poor highly imbalanced solutions. For this reason conditions \eqref{eq:descreasing1}- \eqref{eq:decreasing2} are enabled only from a certain $k \geq Q$.

At the same time, as the algorithm progresses, from efficiency reason it is important to favor the first scenario which accelerates convergence by applying the optimization algorithm to the original objective function. This is automatically induced by the Algorithm NOME, as after a finite number of inner iterations the algorithm never enters in the second scenario. Indeed, at each macro iteration $it$ the threshold value $\bm{\epsilon}_1$ is updated as $\bm{\epsilon}^{it}_1 = \zeta\bm{\epsilon}_1$ with $\zeta \in (0,1)$. As a consequence, after $it$ macro iterations, the maximum number of data points considered by the logic condition $(\bm{\epsilon_1}|I| \geq 1)$ required to enter in the second scenario (see the first \textbf{if} statement of Algorithm \eqref{alg:updatebranching}) is equal to $|I| \bm{\epsilon}^0_1\zeta^{it}$. We simply need to impose $$|I| \bm{\epsilon}^0_1\zeta^{it} \leq 1$$ so that the condition is no longer satisfied. By simple algebra we have $it \geq \frac{ln(|I|\bm{\epsilon}^0_1)}{-ln(\zeta)}.$ Since for each macro iteration $it$, $2^{D-1}$ inner iterations are performed, rounding to the higher integer we have that after at most
$\bar{k} = {\Big \lceil} \frac{ln(|I|\bm{\epsilon}^0_1)}{-ln(\zeta)}{\Big \rceil} 2^{D-1}$ inner iterations the algorithm considers only the first scenario.







\begin{algorithm}[H]
\caption{Update Branch Node}
\label{alg:updatebranching}
$\bm{Input}:t \, branching\,node;\,W^k_B\, working \, set;\, previous\;solution\, \bm{\w}^{k-1}_{{\cal C}_{B}(t)};\, training\,data \, \bm{X};\,\bm{\epsilon_{1}};\,\bm{\epsilon_{2}};\,\bm{\epsilon_{3}}.\\$ 
$\bm{Output}:\,optimal\, values\, \hat{\bm{\w}}_{W^k_B}.$
  
  {\fontsize{10}{12}\selectfont
  \begin{algorithmic}[1]
    
    \Procedure{UpdateBranchNode}{$t,W^k_B,\bm{\w}^{k}_{{\cal C}_{B}(t)},\bm{X},\bm{\epsilon_{1}},\bm{\epsilon_{2}},\bm{\epsilon_{3}}$}
        %\ifthenelse{}{}{}
        \If{($\frac{|I_{left_{t}}|}{|I_{t}|} \leq \bm{\epsilon_{1}}\; \textbf{or}\; \frac{|I_{left_{t}}|}{|I_{t}|} \geq 1 - \bm{\epsilon_{1}}) \;\textbf{and}\;(\bm{\epsilon_1}|I| \geq 1)$ }\Comment{unbalanced instances in children}
        \State $\hat{\bm{\w}}_{W^k_B \setminus t} \gets \bm{\w}^{k}_{{\cal C}_{B}(t) \setminus t}$
            
            \If{$\frac{|I_{left_{t}}|}{|I_{t}|} \leq \bm{\epsilon_{2}}\;\textbf{or}\;\frac{|I_{left_{t}}|}{|I_{t}|} \geq 1 - \bm{ \epsilon_{2}}$}\Comment{worse unbalance}
            
        \State   $\bullet$  set $c_{max} = \argmax\limits_{left_t,right_t}\{|I_{left_{t}}|,|I_{right_{t}}|\}$, $c_{min} = \argmin\limits_{left_t,right_t}\{|I_{left_{t}}|,|I_{right_{t}}|\}$
        \State $\bullet$ move $|I_{c_{max}}|\cdot \bm{\epsilon_{3}}$ data points in $c_{max}$ with largest error \eqref{eq:partial_objective} to $c_{min}$
        \State
        $\bullet$ determine $\hat{\bm{\w}}_{t}$ by optimizing the BLR function \eqref{eq:reshuffle}
        
            \Else
            \State determine $\hat{\bm{\w}}_{t}$ by optimizing the BLR function \eqref{eq:reshuffle}
            \EndIf
            \State $\hat{\bm{\w}}_{W^k_B} \gets \{\hat{\bm{\w}}_{t},\hat{\bm{\w}}_{W^k_B \setminus t} \}$
        \Else
            \State $\hat{\bm{\w}}_{W^k_B} \gets OptmizeBranchingNode(W^k_B,\bm{\w}^{k-1}_{{\cal C}_{B}(t)})$\Comment{optimization with \textit{\textbf{m}} number of iterations} 
        \EndIf
        
        \State \textbf{return} $\hat{\bm{\w}}_{W^k_B}$
 \EndProcedure
  \end{algorithmic}
  }
\end{algorithm} 
 
 
 
 \subsection{Initialization strategy}\label{subsec:init}
%Looking carefully at the objective function \ref{eq:obj}, it is easy to see that the problem we are dealing with is highly nonconvex and therefore very sensitive to starting points. An appropriate choice of starting points can not only facilitate the training phase but also generate solutions with a better generalization error. 

\textcolor{blue}{It is easy to see that the formulation \ref{eq:obj} is very sensitive to starting points due to is highly nonconvex nature. An appropriate choice of starting points can help the training phase and yield solutions with a better generalization error.}


%To propose a meaningful and useful initialization, we must consider the nature of the problem we are dealing with. A decision tree %is nothing more than a%
%\textcolor{blue}{actually performs a recursive partition of the feature space, hence it divides the data points into subgroups.}

%\textcolor{red}{To devise an effective initialization, we must consider the problem nature: decision trees recursively partition the feature space dividing data into subgroups.}


\textcolor{blue}{The idea for our initialization strategy is to exploit a clustering algorithm to induce a recursive partition of the feature space capable of effectively dividing the data points. Starting from the root node with a single cluster composed of all data points we recursively split the top-level cluster into two sub-clusters so as to have for each leaf node at depth $D$ a distinct cluster.}

\textcolor{blue}{Given $I_t$ as the set of data points falling into branch node $t \in \tau_B$, $I_{left_t}$ and $I_{right_t}$ (i.e. set of data points assigned to its left and right children nodes) are determined by clustering $I_t$ into two clusters. This procedure ensures that clustering at node $t$ is applied only
after having applied it to its anchestor node.}



\textcolor{blue}{Since the initialization procedure may exhibit variability due to the randomness inherent in the clustering method, the initialization procedure is repeated over $v$ trials. In our work, we employ the well-known \textbf{K-means} algorithm \cite{lloyd1982least} with \textit{K-means++} random initialization \cite{arthur2007k}.} 

\textcolor{blue}{For each trial $j = 1,\dots,v$, let $A_{\tau_B\cup\tau_L}^j$ be the assignment of data points to every node of the tree, and $A_{\tau_L}^j \subset A_{\tau_B \cup\tau_L}^j$ be the final partition of all data points into the leaf nodes. At the end of each trial $j$, a silhouette score $Sil(A_{\tau_L}^j)$ is computed on the final partition $A_{\tau_L}^j$ to measure the quality of a given clustering. The assignment with the best silhouette score is selected for the initialization.  In our implementation we consider as silhouette score the Davies-Bouldin index \cite{davies1979cluster} which expresses the average similarity measure of each cluster with its most similar cluster.} 




%Since the clustering is in turn affected by randomness, the initialization procedure is repeated in $v$ trials. For each trial $j = 1,\dots,v$, let $A_{\tau_B,\tau_L}^j$ be the assignment of data points to every node of the tree, and $A_{\tau_L}^j \subset A_{\tau_B,\tau_L}^j$ be the final partition of all data points into the leaf nodes. At the end of trial $j = 1,\dots,v$, a silhouette score, which is a measure of the quality of a given clustering \cite{}, is computed on the final partition $A_{\tau_L}^j$, and it is denoted as $Sil(A_{\tau_L}^j)$. Then the assignment achieving the best silhouette score is the candidate for the initialization. 


 

The general scheme of the initialization procedure is given in Algorithm \ref{alg:init}. It is important to notice that for both the clustering method and silhouette score many alternatives can be considered. 













 
 
\begin{algorithm}[h]
\caption{Initialization strategy algorithm}
\label{alg:init}
$\bm{Input}:depth \,\bm{D}; \,iterations\, \bm{v}; dataset\, \bm{I}.\\\bm{Output}:\,assignment\,with\,data\,points\,associated\,to\,leaf\,nodes\,{A_{\tau_L}^{j}}^*. $
  
  {\fontsize{10}{12}\selectfont
  \begin{algorithmic}[1]
    \Procedure{InitializationStrategy}{$\bm{D},\bm{v},\bm{I}$}
    
    \State $DB^{*} \gets BigM$ \Comment{setting big value for the index}
    	\For{$ j = 1,...,\bm{v} $}\Comment{loop over the iterations}
    	\State $A_{\tau_B \cup\tau_L}^j \gets \{\{\bm{I}\}\}$ 
    	\State $A_{\tau_L}^j \gets \{\}$
    	
    		\For{$t = 1,...,2^{D-1} QUIIIIII $}
    		\State $I_{left_{t}},I_{right_{t}} \gets \textrm{K-means}(I_t,n\_clusters=2)$
    		\State $A_{\tau_B\cup\tau_L}^j \gets A_{\tau_B\cup\tau_L}^j \cup \{I_{left_{t}}\} \cup \{I_{right_{t}}\} $
    		\If{$t \geq 2^{D-2} QUIIIIIIII$}
    		\State $A_{\tau_L}^j \gets A_{\tau_L}^j \cup \{I_{left_{t}}\} \cup \{I_{right_{t}}\} $
    		\EndIf
    		\EndFor
    		
    	\State $DB \gets Davies–Bouldin(A_{\tau_L}^j)$\Comment{index of last level nodes}
    	\If{$DB < DB^{*}$}
    	      \State $DB^{*} \gets DB$
    	      \State ${A_{\tau_L}^{j}}^* \gets A_{\tau_L}^j$

    	\EndIf
    	
    	\EndFor
    \State \textbf{return} ${A_{\tau_L}^{j}}^*$
    \EndProcedure
  \end{algorithmic}
  }
\end{algorithm}
 
\subsection{Preliminary analysis}
\label{sec:preliminary_ex}
In this subsection, we summarize preliminary experiments to assess the significance of incorporating heuristics within the NOME decomposition scheme. Firstly, we present results obtained on a synthetic dataset to emphasize the benefits of the reassignment heuristic. Then, we compare the performance of the plain decomposition method to that of decomposition combined with only the reassignment heuristic, as well as with both the reassignment and initialization heuristics, using 4 representative datasets. 

For all the experiments the performance are evaluated by means of a k-fold cross validation with k = 4 and for each fold 20 distinct starting points are generated either randomly or through the initialization procedure when it's included.

To assess the routing capabilities of the decomposition algorithm with the reassignment heuristic versus the plain decomposition, we create a synthetic dataset. This dataset is structured into four clusters, each corresponding to a leaf node in a tree of depth $D=2$. Further information about dataset generation are reported in Appendix \ref\label{appendix:preliminary}.




Figure \ref{fig:gini} presents the Gini index distribution for both the plain decomposition and the decomposition with the reassignment heuristic on the synthetic dataset. Since we know which cluster each data point belongs to, the Gini index helps us determine which method routes data points more accurately. As it is easy to see, the decomposition with the reassignment heuristic is much more capable in routing data points to their respective leaf nodes, often achieving a Gini index of zero, indicating a perfect routing. 

\begin{figure}[h]
    \centering
    \includegraphics[width=0.65\textwidth]{images/Gini_nuovo2.png}
    \caption{Occurences of the Gini index on different runs for plain decomposition and decomposition+reassignment.}
    \label{fig:gini}
\end{figure}

A second set of experiments was conducted on 4 representative datasets, varying in data points and predictor variables, to compare plain model optimization (without decomposition) with incremental introduction of decomposition and the two aforementioned heuristics. Table \ref{table:confrontoalgo} reports the performance in terms of average testing $R^2$, standard deviation, computational training time, and occurrences of producing a senseless model with a negative $R^2$. 

It is easy to see that a plain decomposition method significantly reduces training times compared to plain optimization, but incorporating the heuristics not only improves accuracy but also keeps training times low. In addition, the initialization procedure allows for even better accuracy and it is able to reduce the dependence on starting points (lower standard deviation). 



\begin{table}[h]
\centering
\resizebox{1\columnwidth}{!}{
\begin{tabular}{lcccccccc}
\cline{2-9}
                                             & \multicolumn{4}{c}{Housing}                                                               & \multicolumn{4}{c}{Airfoil-self-noise}                                                    \\ \cline{2-9} 
                                             & Testing $R^2$  & Standard deviation   & Time                 & Anomaly              & Testing $R^2$  & Standard deviation   & Time                 & Anomaly              \\ \hline
plain optimization                      & 0.7142               & 0.0553               & 6.326                & 0                    & 0.5126               & 0.0153               & 2.62                & 1                    \\
plain decomposition                      & 0.7143               & 0.0553               & 1.04                 & 0                    & 0.512                & 0.0157               & 2.35                 & 0                    \\
decomposition+reassignment                            & 0.8094               & 0.088               & 1.79                 & 0                    & 0.7354               & 0.0538               & 3.34                 & 0                    \\
decomposition+reassignment+initialization & 0.849                & 0.041                & 2.87                 & 0                    & 0.759                & 0.0323                & 5.12                & 0                    \\ \hline
                                             & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \cline{2-9} 
                                             & \multicolumn{4}{c}{Ailerons}                                                              & \multicolumn{4}{c}{Puma}                                                                  \\ \cline{2-9} 
                                             & Testing $R^2$  & Standard deviation   & Time                 & Anomaly              & Testing $R^2$  & Standard deviation   & Time                 & Anomaly              \\ \hline
plain optimization                      & 0.8112               & 0.00594              & 537.6              & 40                   & 0.2157               & 0.03069              & 67.9                & 1                    \\
plain decomposition                      & 0.8227               & 0.0044               & 24.72                 & 20                   & 0.2152               & 0.031                & 23.7                & 0                    \\
decomposition+reassignment                           & 0.8324               & 0.0078               & 15.62                & 0                    & 0.7352               & 0.1336               & 39.45               & 0                    \\
decomposition+reassignment+initialization & 0.8324               & 0.006436             & 17.76                & 0                    & 0.813              & 0.0096               & 46.34               & 0                    \\ \hline
\end{tabular}
}
\caption{The results in terms of testing $R^2$, standard deviation, computing time and number of anomalies for 4 datasets (Airfoil, Ailerons, Housing and Puma). Each row represents the steps taken from the first (optimization with a off the shelf solver) to the last (our decomposition method with reassignment and initialization strategy)}
\label{table:confrontoalgo}
\end{table}

Finally to assess the effectiveness of our initialization procedure with the selection of the best Davies-
Bouldin index, we have also tested the algorithm \ref{alg:init} and decomposition method on the Housing dataset. See Appendix \ref{appendix:preliminary} for more details.



==> sections/implementation_previous_old.tex <==
\section{Practical implementation}\label{subsec:implementation}
In this section we present the implemented decomposition algorithm, the so-called NOME, which is a version of the NDGS general algorithm presented in Section \ref{subsec:scheme}. Indeed, NOME alternates a nonconvex optimization with respect to the branching node variables (\textbf{BN Step}), with a convex optimization with respect to a subset of leaf node variables (\textbf{LN Step}).

Although being asymptotically convergent according to theory presented in Section \ref{subsec:convergence}, NOME embeds in the first steps two heuristic procedures: a clustering-based initialization, and a samples reassignment procedure. Such heuristics are helpful in reducing instability phenomena, in particular early convergence to poor solutions and degenerate routing of almost all samples towards a single path in the tree,  which often affect the training of (randomized) regression trees. \textcolor{red}{The main reason for these poor solutions is the high complexity of the objective function. Indeed, in addition to the problems of least squares associated to each leaf nodes, the problem of routing and assigning instances in the branching nodes turns out to be highly difficult to handle with a generic solver. The previous drawbacks favour the occurrence of failures in which negative $R^2$ are obtained, referred here as ``\textit{anomalies}"}. 

In this introduction we show preliminary experiments providing the flavor of the importance of embedding the heuristics in the proposed decomposition method. In particular, we firstly present some results obtained on a synthetic dataset to highlight the benefits of the reassignment heuristic, then we compare the performance of the plain decomposition with respect to the decomposition combined with the sole reassignment heurisitic an both reassignment and initialization heuristics on 4 representative datasets. 

The synthetic dataset is composed by 1500 data points structurally clustered into four clusters so that, in principle, each distinct cluster can be identified by one of the four leaf nodes of a tree at depth 2. The left side of Figure \ref{fig:sfig1} shows the 3D plot for the input vectors, while for the output response we define distinct coefficients and an equal white noise of zero mean and 0.1 standard deviation.
\begin{figure}[h] 
    \centering
    %\subfloat[data a]{%
        \includegraphics[width=0.5\textwidth]{images/sintetico_nuovo}%
        \label{fig:sfig1}%
        %}%
    \hfill%
    %\subfloat[data b]{%
        \includegraphics[width=0.5\textwidth]{images/Gini_nuovo.png}%
        \label{fig:b}%
        %}%
    \caption{On the left the 3D representation of the 4 clusters of the synthetic dataset. On the right the histogram of the distributions of the Gini index value on different runs for plain decomposition (green) and decomposition + reassignment (blue). }
\end{figure}

The aim is to compare the routing capabilities of the decomposition algorithm embedded with the reassignment heuristic with a plain decomposition version. To do so, we use the Gini index to measure the effectiveness of the  cluster assignment to leaf nodes. By knowing which cluster each data point belongs to, the Gini index let us know which of the two methods is more suitable at routing instances correctly. 
The training Gini index is evaluated by means of a k-fold cross validation with k= 4. For each fold we train the model starting from 20 distinct random starting points. The right side of Figure \ref{fig:b} presents the distribution of the Gini index for both the plain decomposition and the decomposition with the reassignment heuristic. 
As it is easy to see, the latter version is much more capable to route data points to the appropriate leaf node associated to its related cluster. In some cases it is able to achieve a Gini index equal to zero by distributing each data point without errors. %This behavior is confirmed by the results related to the algoritmo proposto and semplice decomposizione in Table \ref{table:confrontoalgo}. While a slight improvement in terms of accuracy and stability (i.e., fewer anomalies) is achieved, the results remain lower in terms of out-of-sample $R^2$ than the algoritmo proposto. It is important to note how the decomposition is able, compared to simple optimization, to drastically reduce computation times.
\par 
A second set of experiments is performed on 4 representative datasets, distinguished by number of data points and predictor variables, and it compares the plain optimization of model?? with the incremental introduction of the decomposition and the two aforementioned heuristics. Results, reported in Table \ref{table:confrontoalgo}, are measured in terms of average out-of-sample $R^2$, standard deviation, computational training time, and number of anomalies. %(i.e. number of times in which a senseless model with a negative $R^2$ is provided). 
 The testing results are evaluated by means of a k-fold cross validation with k= 4. In this way every subset of the dataset is treated as a testing set, whereas the rest is involved in the training of the model. Then the average of the resulting k accuracy estimations is taken as an estimate of the model accuracy. For each fold we train the model starting from 20 distinct random starting points.
\par It is easy to see how a plain decomposition method is able to substantially reduce the training times \textcolor{red}{with respect to the plain optimization}, %without changing significantly the accuracy
 while embedding the heuristics allows to obtain a good trade-off between accuracy and training times.\par

\begin{table}[h!]
\centering
\resizebox{1\columnwidth}{!}{
\begin{tabular}{lcccccccc}
\cline{2-9}
                                             & \multicolumn{4}{c}{Housing}                                                               & \multicolumn{4}{c}{Airfoil-self-noise}                                                    \\ \cline{2-9} 
                                             & Out-of-sample $R^2$  & Standard deviation   & Time                 & Anomaly              & Out-of-sample $R^2$  & Standard deviation   & Time                 & Anomaly              \\ \hline
plain optimization                      & 0.7142               & 0.0553               & 6.326                & 0                    & 0.5126               & 0.0153               & 2.62                & 1                    \\
plain decomposition                      & 0.7143               & 0.0553               & 1.04                 & 0                    & 0.512                & 0.0157               & 2.35                 & 0                    \\
decomposition+reassignment                            & 0.8094               & 0.088               & 1.79                 & 0                    & 0.7354               & 0.0538               & 3.34                 & 0                    \\
decomposition+reassignment+initialization & 0.849                & 0.041                & 2.87                 & 0                    & 0.759                & 0.0323                & 5.12                & 0                    \\ \hline
                                             & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \cline{2-9} 
                                             & \multicolumn{4}{c}{Ailerons}                                                              & \multicolumn{4}{c}{Puma}                                                                  \\ \cline{2-9} 
                                             & Out-of-sample $R^2$  & Standard deviation   & Time                 & Anomaly              & Out-of-sample $R^2$  & Standard deviation   & Time                 & Anomaly              \\ \hline
plain optimization                      & 0.8112               & 0.00594              & 537.6              & 40                   & 0.2157               & 0.03069              & 67.9                & 1                    \\
plain decomposition                      & 0.8227               & 0.0044               & 24.72                 & 20                   & 0.2152               & 0.031                & 23.7                & 0                    \\
decomposition+reassignment                           & 0.8324               & 0.0078               & 15.62                & 0                    & 0.7352               & 0.1336               & 39.45               & 0                    \\
decomposition+reassignment+initialization & 0.8324               & 0.006436             & 17.76                & 0                    & 0.813              & 0.0096               & 46.34               & 0                    \\ \hline
\end{tabular}
}
\caption{The results in terms of testing $R^2$, standard deviation, computing time and number of anomalies for 4 datasets (Airfoil, Ailerons, Housing and Puma). Each row represents the steps taken from the first (optimization with a off the shelf solver) to the last (our decomposition method with reassignment and initialization strategy)}
\label{table:confrontoalgo}
\end{table}

The remainder of this section is organized as follows. In Section \ref{subsec:algorithm} algorithm NOME is described in detail together with all convergence aspects, Section \ref{subsec:reass} is devoted to the description of the reassignment heuristic, while Section \ref{subsec:init} describes the initialization strategy.


\subsection{The algorithm description}\label{subsec:algorithm}
Before presenting the details of algorithm NOME, it is necessary to comment on a crucial aspect concerning the "nonconvex" \textbf{BN Step}. As highlighted in Section \ref{subsec:convergence}, to prevent oscillating behaviour of the decomposition method and to ensure asymptotic convergence it is important to satisfy \textbf{Condition} \ref{con:2} in the \textbf{BN Step} update. This can be easily obtained by using the partial steepest descent direction in tandem with the well-known Armijo method (see e.g., Bertsekas \cite{Bertsekas/99}). That is, given $W^k_B$, then $\bm{\w}_{W^k_B}^{k+1}$ is set equal to the following Armijo update

\begin{equation}
\label{eq:steepest}
  \bm{\w}_{W^k_B}^{k} + \alpha^k_{W^k_B} \bm{d}_{W^k_B}^k,
\end{equation}


\noindent where $\bm{d}_{W^k_B}^k = - \nabla_{\bm{\w}_{W^k_B}}E(\bm{\w}^k,\bm{\beta}^k)$, and the step length $\alpha^k_{W^k_B}$ is computed through Algorithm \ref{alg:Armijo} reported below, starting from an initial guess $a > 0$.

\begin{algorithm}[H]
\caption{Armijo method}
\label{alg:Armijo}
$\bm{Input}: a\,>\,0;\, \gamma\, \in\, (0,1);\, \delta\,\in\,(0,1);\,(\bm{\w},\bm{\beta});\,J\\$ 
$\bm{Output}:\alpha_J.$
{\fontsize{10}{12}\selectfont
\begin{algorithmic}[1]
\Procedure{ArmijoMethod}{$a,\gamma,\delta,(\bm{\w},\bm{\beta}),J$}
\State $\alpha \gets a$
\While{$ E(\bm{\w}_{J} + \alpha \bm{d}_{J},\bm{\w}_{\bar J},\bm{\beta}) < E(\bm{\w},\bm{\beta}) -\gamma \alpha \|\nabla_{J}E(\bm{\w},\bm{\beta}) \|^2 $}
\State $\alpha \gets \delta \alpha$

\EndWhile
\State $\alpha_J \gets \alpha$
\State \textbf{return} $\alpha_J$
\EndProcedure
\end{algorithmic}
}
\end{algorithm}


By adapting the result proved in Grippo et al. \cite{grippo2015decomposition} to our MRRT framework, it is possible to state some theoretical properties of Algorithm \ref{alg:Armijo} needed for the asymptotic convergence of Algorithm NOME (stated in Proposition \ref{prop:prop3}) and reported in the next proposition, whose proof can be found in Appendix.

\begin{proposition}
\label{prop:prop2}
Let $J \subseteq \tau_B$ be a fixed set of indices and let  $\{(\bm{\w}^k,\bm{\beta}^k)\}_K$ be an infinite subsequence such that $$\nabla_{J} E(\bm{\w}^k,\bm{\beta}^k) \neq 0 $$ and assume that, for all $k \in K$, the step length $\alpha^k_{J}$ is calculated by Armijo method procedure \ref{alg:Armijo} along the direction $\bm{d}_{J}^k = - \nabla_J E(\bm{\w}^k,\bm{\beta}^k)$.

Then, the algorithm terminates yielding a stepsize $\alpha^k_{J} > 0$ such that the following hold.
\begin{enumerate}
    \item[(i)] For all $k \in K$, we have
    \begin{equation}
        E(\bm{\w}_{J}^{k} + \alpha^k_{J} \bm{d}_{J}^k,\bm{\w}_{\bar J}^k,\bm{\beta}^k) < E(\bm{\w}^k,\bm{\beta}^k)
    \end{equation}
    \item[(ii)] If the following limit is valid:
        \begin{equation}
            \lim\limits_{k \to \infty. k \in K} E(\bm{\w}^k,\bm{\beta}^k) - E(\bm{\w}_{J}^{k} + \alpha^k_{J} \bm{d}_{J}^k,\bm{\w}_{\bar J}^k,\bm{\beta}^k)=0
        \end{equation}
        then 
            \begin{enumerate}[label={\alph*)}]
            \item $ \lim\limits_{k \to \infty. k \in K} \alpha^k_{J} \|\bm{d}^k_{J} \|=0$.
            \item If $\{(\bm{\w}^k,\bm{\beta}^k)\}_{K_1},\, K_1 \subseteq K$ is a convergent subsequence, we have 
            \begin{equation}
                \lim\limits_{k \to \infty. k \in K_1} \nabla_{J}E(\bm{\w}^k,\bm{\beta}^k)=0.
            \end{equation}
            \end{enumerate}
\end{enumerate}
\qedblack
\end{proposition}



 At the \textbf{BN Step}, the Armijo update acts as a reference point if a different method is used to determine $\bm{\w}_{W^k_B}^{k+1}$. Let us denote the Armijo update computed as in \eqref{eq:steepest} as $\bm{\w}^{ref}_{W^{k}_B}$, and the alternative candidate point as $\hat{\bm{\w}}_{W^k_B}$. If we set $\bm{\w}_{W^k_B}^{k+1}=\hat{\bm{\w}}_{W^k_B}$, then convergence is ensured provided the following two conditions are satisfied  
\begin{equation}
\label{eq:descreasing1}
    E(\hat{\bm{\w}}_{W^k_B}^k,\bm{\w}_{\bar W^k_B}^k,\bm{\beta}^k) \leq E(\bm{\w}^{ref}_{W^{k}_B},\bm{\w}_{\bar W^k_B}^{k},\bm{\beta}^k),
\end{equation}
and
\begin{equation}
\label{eq:decreasing2}
    E(\hat{\bm{\w}}_{W^k_B}^k,\bm{\w}_{\bar W^k_B}^k,\bm{\beta}^k) \leq E(\bm{\w}^k,\bm{\beta}^k) - \tau \|\hat{\bm{\w}}_{W^k_B}^k - \bm{\w}_{W^k_B}^k \|^2,
\end{equation}

for a given $\tau > 0$. Condition \eqref{eq:decreasing2} is necessary to guarantee that the convergence of the function values implies $\| \bm{\w}_{W^k_B}^{k+1} - \bm{\w}_{W^k_B}^{k}\| \to 0$, which for the Armijo point $\bm{\w}^{ref}_{W^k_B}$ is automatically enforced by $(ii)- a)$ in Proposition \ref{prop:prop2}.\par 
Now, we are ready to present the decomposition method NOME, whose scheme is reported in Algorithm \ref{alg:Decomposition1}. After initializing the starting solution $(\bm{\w^0},\bm{\beta^0})$ via the $\textsc{InitializationStrategy}$ procedure (described below in Section \ref{subsec:init}), the algorithm is structured as a main external loop of macro iterations, indicated by variable $it$ and iterated until a generic termination test is verified. At each macro iteration $it$, an internal loop of inner iterations $k$ iteratively selects a branching node $t\in \tau_B$ at a time to construct the working set. In particular, $t$ and the set of indices of its branching node descendants (denoted as ${\cal C}_B(t)$) are inserted in $W_B$. Similarly, $W_L$ is defined as the set of all indices of leaf nodes which are descendant of $t$ (denoted as ${\cal C}_L(t)$). The only exception is when $t$ is the root node and $D > 1$. In this case $W_B \equiv \{t\}$ and $W_L \equiv \emptyset$. Once determined $W_B$ and $W_L$, \textbf{BN Step} and \textbf{LN Step} are sequentially performed.

Regarding the $\textbf{BN Step}$, the branching node variables subvector $\bm{\w}_{W^k_B}$ is actually updated only if the norm of the partial gradient $\| \nabla_{{W^k_B}}E(\bm{\w}^k,\bm{\beta}^k)\|$ is greater than a certain decreasing threshold $\theta_{\w}^k$. In such a case, a reference update subvector $\bm{\w}_{W^k_B}^{ref}$ is computed by means of % a s a step $\alpha_{W^k_B}^k$ along the partial antigradient direction $\nabla_{W^k_B}E(\bm{\w}^k,\bm{\beta}^{k})$, where $\alpha_{W^k_B}^k$ is determined by a standard Armjio linesearch step (see e.g., Bertsekas \cite{Bertsekas/99}) through the \textsc{ArmijoMethod} procedure.
the Armijo linesearch described above.
%As detailed in Section \ref{subsec:pract-theo}, the Armijo reference point is used both as a practical guide to prevents oscillation during the iteration progress, and to ensure theoretical asymptotic convergence. 
Then, %for $k \leq Q$ (where $Q$ is a positive integer set by the user),
the \textsc{UpdateBranchNode} procedure (described in detail in Section \ref{subsec:reass}) computes a new candidate point $\hat{\bm{\w}}_{W^k_B}$ either by any standard unconstrained minimization algorithm, or by a specific heuristic method allowing to induce balancing of data distribution within the branching nodes whenever data are particularly imbalanced. The data imbalance tolerance is handled by the thresholds $\bm{\epsilon}_1, \bm{\epsilon}_2 \,\text{and}\, \bm{\epsilon}_3$.  %This second possibility is considered when certain conditions related to the balancing of the instances within the block are met. 
The heuristic method is helpful to improve stability during the initial stages of the algorithm. At the same time to ensure convergence for sufficiently large $k$ (i.e., $k > Q$ where $Q$ is a positive integer set by the user) the new point will be taken only if it satisfies conditions \eqref{eq:descreasing1} and \eqref{eq:decreasing2}, otherwise Armijo reference update is taken (see Steps 17-20).

Also the \textbf{LN Step} is actually performed only if the norm of the partial gradient $\| \nabla_{{W^k_L}}E(\bm{\w}^{k+1},\bm{\beta}^k) \|$ is greater than $\theta_{\beta}^k$. The optimization of the leaf node variables subvector $\bm{\beta}_{W^k_L}^{k}$ corresponds to a linear least-squares problem thus we can minimize it either through an iterative method for convex quadratic function or by a direct method for the linear least-squares problem.

\textcolor{blue}{Notice that for both \textbf{BN Step} and \textbf{LN Step}, whenever $k \leq Q$, no specific restrictions are imposed for the updates $\bm{\w}_{W^k_B}^{k+1}, \bm{\beta}_{W^k_L}^{k+1}$. Among many possible choices, this methodological freedom allows to take into account only a subset of data points in the resolution of each subproblem so as to speed up the first iterations. In particular, in our implementation, for a given current node $t$ we consider only data points falling into $t$ with a probability larger than 0.5 in the optimization problems related to the \textbf{BN Step} and \textbf{LN Step}, as these points are considered more ``relevant" when determining variables involved in sets $W_B^k$ and $W_L^k$ induced by $t$. Notice that this specific choice should be not confused with a mini-batch sample-based decomposition approach (see e.g.,[]), as the number of samples falling into a node with a certain probability cannot be controlled a priori.}

At the end of each inner iteration the parameters $\bm{\epsilon}_1, \bm{\epsilon}_2 \,\text{and}\, \bm{\epsilon}_3$ controlling the data imbalance are decreased. As it will be specified in the \textsc{UpdateBranchNode} scheme, the smaller are these parameters the more data imbalance is allowed. 

\begin{algorithm}[h]
\caption{Decomposition algorithm}
\label{alg:Decomposition1}
$\bm{Input}: depth \,\bm{D}; training\,data \, \bm{X},\bm{y};\,max\,iterations\,\bm{Max\_iter}; \bm{\epsilon_{1}}^0,\,\bm{\epsilon_{2}}^0,\,\bm{\epsilon_{3}}^0,\,\bm{\zeta},\,\theta_{\w},\, \theta_{\beta} \in [0,1)\,$ 
%\vspace{-5pt}
$\\ with\, \bm{\epsilon_{1}}\, >\,\bm{\epsilon_{2}};\,\upsilon \in [0,1);\, Q \in \mathbb{N}, \tau>0.$ 
%\vspace{-10pt}
$\\ \bm{Output}:\,optimal\, values\, \bm{\w^{*}},\,\bm{\beta^{*}}.$
\vspace{-10pt}
  {\fontsize{10}{12}\selectfont
  \begin{algorithmic}[1]
  \Statex {} 
    \State $(\bm{\w}^{0},\bm{\beta}^{0}) \gets\textsc{InitializationStrategy}(\bm{D},\bm{v},\bm{X})$
    \Procedure{Decomposition}{$\bm{D},\bm{X},\bm{y},\bm{\w^0},\bm{\beta^0},\bm{\epsilon_{1}},\bm{\epsilon_{2}},\bm{\epsilon_{3}},\bm{\gamma},\theta_{\w},\theta_{\beta},\upsilon$}
      
      \State $\bullet$ $(\bm{\w}^{*},\bm{\beta}^{*}) \gets \bm{\w}^{0},\bm{\beta}^{0}$
      \State $\bullet$ $\bm{\epsilon_{1}},\,\bm{\epsilon_{2}},\,\bm{\epsilon_{3}}\gets \bm{\epsilon_{1}}^0,\,\bm{\epsilon_{2}}^0,\,\bm{\epsilon_{3}}^0$
      \State $\bullet$ $error_{best} \gets E(\bm{\w}^{*},\bm{\beta}^{*})$
      \State $\bullet$ $k \gets 0,\, it \gets 1,$
      \While{$ it < \bm{Max\_iter}\,and\,$ not {\it termination test}}
       
        \For{$ t = 1,...,2^{\bm{D}}-1 $}\Comment{loop over the branching nodes}
        
        \If{$t == 1\,\text{and}\, \bm{D} > 1$}
        \State $W^k_B \gets \{t\}, \, W^k_L \gets \emptyset$
        \Else
        \State $W^k_B \gets \{t,{\cal C}_{B}(t)\}, \, W^k_L \gets {\cal C}_{L}(t)$
        \EndIf
        
        %\State $W^k_B \gets \{t\}, \, W^k_L \gets children_leaf(t)$
       \Statex
        \Statex  {$\triangleright$ \, \textbf{BN Step}} \textit{(Optimization of branching nodes parameters)}
        
        \If{$\| \nabla_{{W^k_B}}E(\bm{\w}^k,\bm{\beta}^k) \| \leq (\theta_{\w})^k$}
        \State $\bm{\w}^{k+1}\gets \bm{\w}^{k}$
        \Else
        \State $\bullet$ $\alpha_{W^k_B}^k \gets \textsc{ArmijoMethod}(a,\gamma,\delta,(\bm{\w}^{k},\bm{\beta}^k),W^k_B)$
        \State $\bullet$ $\bm{\w}_{W^k_B}^{ref} \gets \bm{\w}_{W^k_B} - \alpha_{W^k_B}^k \nabla_{W^k_B}E(\bm{\w}^k,\bm{\beta}^{k})$
        \State $\bullet$ $\hat{\bm{\w}}_{W^k_B} \gets $\textsc{UpdateBranchNode}$(t,W^k_B,\bm{\w}^{k}_{W^k_B},\bm{X},\bm{\epsilon_{1}},\bm{\epsilon_{2}},\bm{\epsilon_{3}})$ %\Comment{technique that   satisfies }
        
        
            
            
        \If{($\hat{\bm{\w}}_{W^k_B}$ satisfies \eqref{eq:descreasing1}- \eqref{eq:decreasing2}) or ($k \leq Q $)} 
            \State $\bm{\w}_{W^k_B}^{k+1} \gets \hat{\bm{\w}}_{W^k_B}$
        \Else
            \State $\bm{\w}_{W^k_B}^{k+1} \gets \bm{\w}_{W^k_B}^{ref}$
        \EndIf
        
        
        
        
        
        \EndIf
        
        
        \Statex
        \Statex  {$\triangleright$ \, \textbf{LN Step}} \textit{(Optimization of leaf nodes parameters)}
        
        \If{$\| \nabla_{{W^k_L}}E(\bm{\w}^{k+1},\bm{\beta}^k) \| \leq (\theta_{\beta})^k$}
        \State $\bm{\beta}^{k+1}\gets \bm{\beta}^{k}$
        \Else
        \textcolor{blue}{\If{$k \leq Q $} 
            \State compute $\bm{\beta}_{W^k_L}^{k+1} $ by any method
        \Else
            \State compute $\bm{\beta}_{W^k_L}^{k+1}$ such that \\ \qquad \qquad \qquad \;\;\;\, $E(\bm{\w}^{k+1},\bm{\beta}^{k+1})\leq E(\bm{\w}^{k+1},\bm{\beta}^{k})\; \textbf{and} \; \| \nabla_{W^k_L}E(\bm{\w}^{k+1},\bm{\beta}^{k+1}) \| \leq (\upsilon)^k$
        \EndIf
        }
        
        %\State compute $\bm{\beta}_{W^k_L}^{k+1}$ such that $E(\bm{\w}^{k+1},\bm{\beta}^{k+1}) \leq E(\bm{\w}^{k+1},\bm{\beta}^{k})\; \textbf{and}\; \| \nabla_{W^k_B}E(\bm{\w}^{k+1},\bm{\beta}^{k+1}) \| \leq (\upsilon)^k$ \Statex
        
        \EndIf
        \If{$E(\bm{\w}^{k+1},\bm{\beta}^{k+1})< error_{best}$}
        \State $\bullet$ $error_{best} \gets E(\bm{\w}^{k+1},\bm{\beta}^{k+1})$
        \State $\bullet$ ($\bm{\w}^{*},\bm{\beta}^{*}) \gets (\bm{\w}^{k+1},\bm{\beta}^{k+1})$
        \EndIf
        %\State \texttt{left_{t} = descendant(t,right=\bm{True})}
        \State $k \gets k + 1$
        \EndFor
	  \State $\bullet$ $\bm{\epsilon_{1}},\,\bm{\epsilon_{2}},\,\bm{\epsilon_{3}} \gets \bm{\zeta}\cdot\bm{\epsilon_{1}},\,\bm{\zeta}\cdot\bm{\epsilon_{2}},\,\bm{\zeta}\cdot\bm{\epsilon_{3}}$
	  \State $\bullet$ $it \gets it + 1$
      \EndWhile\label{Decompositiondwhile}
      \State \textbf{return} $(\bm{\w}^{*},\bm{\beta}^{*})$
    \EndProcedure
  \end{algorithmic}
  }
\end{algorithm} 
 



%Thanks to \textbf{Proposition} \ref{prop:prop2} assuming that at each step of the subsequence we apply steepest direction in tandem with Armijo's step length as in \eqref{eq:steepest}, since the stepsize is bounded above, the convergence of the function values implies that the subsequence satisfies $\|\bm{\w}_{W^k_B}^{k+1} - \bm{\w}_{W^k_B}^{k} \| \rightarrow 0$ as $k \to \infty$. 

 

It is important to note that, to preserve asymptotic convergence, it is sufficient to impose conditions \eqref{eq:descreasing1} and \eqref{eq:decreasing2} on $\hat{\bm{\w}}_{W^k_B}^k$ only for sufficiently large $k$.
%After the \textbf{BN Step} phase we obtain a point $(\bm{\w}^{k+1},\bm{\beta}^k)$.


In Proposition \ref{prop:prop3} (whose proof is reported in Appendix) we establish the convergence properties of NOME, assuming that it generates an infinite sequence $\{(\bm{\w}^k,\bm{\beta}^k)\}$ of points.
\begin{proposition}
\label{prop:prop3}
Given an infinite sequence $\{(\bm{\w}^k,\bm{\beta}^k)\}$ generated by Algorithm NOME. The following holds:
\begin{enumerate}[label={\arabic*)}]
    \item $\{(\bm{\w}^k,\bm{\beta}^k)\}$ has a limit points.
    \item The sequence $\{E(\bm{\w}^k,\bm{\beta}^k)\}$ converges to a limit.
    \item We have $\lim\limits_{k \to \infty}\|\bm{\beta}^{k+1} -\bm{\beta}^k\|=0 $
    \item For any $ j \in \tau_B$, we have $$\lim\limits_{k \to \infty}\| \bm{\w}_{j}^{k+1} - \bm{\w}_{j}^{k} \|=0$$
    \item Every limit point of $\{(\bm{\w}^k,\bm{\beta}^k)\}$ is a stationary point of $E(\bm\w,
\bm\beta)$ in \eqref{eq:obj}.
\end{enumerate}
\qedblack
\end{proposition}

\subsection{Optimization strategies in the BN Step}\label{subsec:reass}

During the \textbf{BN Step} of Algorithm \ref{alg:Decomposition1} the new point can be calculated by means of the \textsc{UpdateBranchNode} procedure, whose scheme is reported in Algorithm \ref{alg:updatebranching}. \textsc{UpdateBranchNode} considers two possible scenarios according to how the ancestor node $t$ of $W_B^k$ addresses data points towards its two children nodes: either the distribution of data points is sufficiently uniform between the children nodes, or it is highly imbalanced. 
To this aim, recalling the randomized nature of MRRT, we consider the set of data points falling into the node $t$ and denoted as $I_t$, the one obtained by setting an appropriate threshold on the sigmoid functions in the ancestors node of $t$, therefore simulating a deterministic behavior as done in prediction phase (see \eqref{eq:prediction_model}). Let us also define the two children nodes of $t$ as $left_t$ and $right_t$, and consequentially the subsets of data points falling into these nodes as $I_{left_t}$ and $I_{right_t}$.
In the first scenario, data points are sufficiently balanced, i.e. for a given threshold $\bm{\epsilon_{1}} \in (0,1)$ $\bm{\epsilon_{1}} < \frac{|I_{left_{t}}|}{|I_{t}|} < 1 - \bm{\epsilon_{1}}$. Then, the new candidate point is obtained through any nonlinear unconstrained minimization algorithm (e.g., a Newton, a Quasi-Newton or a conjugate gradient method).

In the second scenario, where $\frac{|I_{left_{t}}|}{|I_{t}|} \leq \bm{\epsilon_{1}}$ or\, $\frac{|I_{left_{t}}|}{|I_{t}|} \geq 1 - \bm{\epsilon_{1}}$, only the variables associated to ancestor $t$ are actually optimized as the aim is solely to improve the balance of data points passing through it. The candidate point is obtained by taking into account the level of imbalance. In particular, if for a given threshold $\bm{\epsilon_{2}} < \bm{\epsilon_{1}}$ we have $\bm{\epsilon_{2}} < \frac{|I_{left_{t}}|}{|I_{t}|} < 1 - \bm{\epsilon_{2}}$, the imbalance is moderate and the variables associated to $t$ are obtained by optimizing (through any unconstrained optimization method as in the first scenario) a proxy of the original objective function based on a Balanced Logistic Regression (BLR) function which tends to improve the balance of data points routed in $t$.
The BLR objective function is as follows:
\begin{equation}
\label{eq:reshuffle}
 -\frac{1}{|I_t|} \sum_{i \in I_t} w_ic_iln(p_{it}(\bm{x}_i)) + w_i(1 - c_i)ln(1-p_{it}(\bm{x}_i))  
\end{equation}


\noindent where $c_i = 0$ and $w_i = \frac{|I_t|}{2|I_{left_t}|}$ if the data point $i\in I_{left_t}$, $c_i = 1$ and $w_i = \frac{|I_t|}{2|I_{right_t}|}$ otherwise.


If $\frac{|I_{left_{t}}|}{|I_{t}|} \leq \bm{\epsilon_{2}}$ or\, $\frac{|I_{left_{t}}|}{|I_{t}|} \geq 1 - \bm{\epsilon_{2}}$, the imbalance is considered strong. Then, the optimization of the BLR function is combined with a prior reassignment heuristic used to force data points balance. The heuristic works by moving a fraction $\bm{\epsilon}_3 \in (0,1)$ of data points from the children node with the largest number of them to the other children node. The reassigned data points are those corresponding to larger error values in the partial objective function related to the subtree with the first ancestor $t$, which are considered the more likely to be addressed in the wrong children node. Formally, for a given data point $i$ its partial error is computed as follows:
\begin{equation}
   \label{eq:partial_objective}
    \sum_{t\in {\cal C }_L(t)}P_{it}(\bm{\w})\cdot(\hat y_{it}(\bm{\beta}_t)-y_{i})^{2}.
\end{equation}
The choice of data points to be moved can be also randomized, but preliminary experiment showed that the residual based selection is more effective.

%Whenever the distribution of data among branching nodes is too imbalanced, the idea is to perturb the data points distribution with a reassignment heuristic. The reassignment heuristic is a procedure to both route the data points in the right subproblem and to balance the distribution of data points among the branching nodes of the subtree. This ensures greater stability in the training phase by directing optimization towards solutions that would otherwise be difficult to achieve.

%Concerning the number of data points involved in each subproblem the proposed algorithm considers only data points that falls into the branching node related to the subproblem. It is possible to establish the instances which fall into the subtree, setting an appropriate threshold on the logistic function in the ancestor node of branching node.

%We need to introduce $\bm{\epsilon}_1$ and $\bm{\epsilon}_2$ which represent different thresholds for the assignment of data points in order to manage the possible data imbalance.
%For each branching node $t$ we identify the indices of the children nodes $I_{left_t}$ and $I_{right_t}$. 
%If the imbalance between the data of the child nodes does not exceed the threshold $\epsilon_1$ we optimize the variables through a convergent technique, otherwise we check if the imbalance is greater than the second threshold $\epsilon_2$.
%If the imbalance between the data of the child nodes does not exceed the threshold $\epsilon_1$ we optimize the subproblem with respect $\bm{\w}_{W^k_B}$ through a unconstrained convergent nonlinear optimization algorithm, otherwise we check if the imbalance is greater than the second threshold $\epsilon_2$. If the imbalance is higher than the threshold $\epsilon_2$ we apply the procedure \textit{BalancedLogisticRegression} with reshuffling, otherwise the procedure \textit{BalancedLogisticRegression} is applied without reshuffling.

It is important to emphasize that in the case where the BLR function is used, it is very unlikely that the two acceptance conditions \eqref{eq:descreasing1}- \eqref{eq:decreasing2} in Algorithm \ref{alg:Decomposition1} will be satisfied, as the problem to be solved is a proxy of the original one. Nonetheless, a periodical optimization of the BLR function provides a very effective stabilization of Algorithm \ref{alg:Decomposition1} during the first macro iterations, avoiding to get stuck in poor highly imbalanced solutions. For this reason conditions \eqref{eq:descreasing1}- \eqref{eq:decreasing2} are enabled only from a certain $k \geq Q$.

At the same time, as the algorithm progresses, from efficiency reason it is important to favor the first scenario which accelerates convergence by applying the optimization algorithm to the original objective function. This is automatically induced by the Algorithm NOME, as after a finite number of inner iterations the algorithm never enters in the second scenario. Indeed, at each macro iteration $it$ the threshold value $\bm{\epsilon}_1$ is updated as $\bm{\epsilon}^{it}_1 = \zeta\bm{\epsilon}_1$ with $\zeta \in (0,1)$. As a consequence, after $it$ macro iterations, the maximum number of data points considered by the logic condition $(\bm{\epsilon_1}|I| \geq 1)$ required to enter in the second scenario (see the first \textbf{if} statement of Algorithm \eqref{alg:updatebranching}) is equal to $N \bm{\epsilon}^0_1\zeta^{it}$. We simply need to impose $$|I| \bm{\epsilon}^0_1\zeta^{it} \leq 1$$ so that the condition is no longer satisfied. By simple algebra we have $it \geq \frac{ln(|I|\bm{\epsilon}^0_1)}{-ln(\zeta)}.$ Since for each macro iteration $it$, $2^{D-1}$ inner iterations are performed, rounding to the higher integer we have that after at most
$\bar{k} = {\Big \lceil} \frac{ln(|I|\bm{\epsilon}^0_1)}{-ln(\zeta)}{\Big \rceil} 2^{D-1}$ inner iterations the algorithm considers only the first scenario

%This aspect is positive in terms of efficiency because it guarantees that by $k \geq Q$ the procedure will apply a convergent method (e.g. Quasi Newton method) that is more likely to satisfy the conditions \eqref{eq:descreasing1}- \eqref{eq:decreasing2} and thus be used instead of the less efficient Armijo method.





\begin{algorithm}[H]
\caption{Update Branch Node}
\label{alg:updatebranching}
$\bm{Input}:t \, branching\,node;\,W^k_B\, working \, set;\, previous\;solution\, \bm{\w}^{k-1}_{{\cal C}_{B}(t)};\, training\,data \, \bm{X};\,\bm{\epsilon_{1}};\,\bm{\epsilon_{2}};\,\bm{\epsilon_{3}}.\\$ 
$\bm{Output}:\,optimal\, values\, \hat{\bm{\w}}_{W^k_B}.$
  
  {\fontsize{10}{12}\selectfont
  \begin{algorithmic}[1]
    
    \Procedure{UpdateBranchNode}{$t,W^k_B,\bm{\w}^{k}_{{\cal C}_{B}(t)},\bm{X},\bm{\epsilon_{1}},\bm{\epsilon_{2}},\bm{\epsilon_{3}}$}
        %\ifthenelse{}{}{}
        \If{($\frac{|I_{left_{t}}|}{|I_{t}|} \leq \bm{\epsilon_{1}}\; \textbf{or}\; \frac{|I_{left_{t}}|}{|I_{t}|} \geq 1 - \bm{\epsilon_{1}}) \;\textbf{and}\;(\bm{\epsilon_1}|I| \geq 1)$ }\Comment{unbalanced instances in children}
        \State $\hat{\bm{\w}}_{W^k_B \setminus t} \gets \bm{\w}^{k}_{{\cal C}_{B}(t) \setminus t}$
            
            \If{$\frac{|I_{left_{t}}|}{|I_{t}|} \leq \bm{\epsilon_{2}}\;\textbf{or}\;\frac{|I_{left_{t}}|}{|I_{t}|} \geq 1 - \bm{ \epsilon_{2}}$}\Comment{worse unbalance}
            
        \State   $\bullet$  set $c_{max} = \argmax\limits_{left_t,right_t}\{|I_{left_{t}}|,|I_{right_{t}}|\}$, $c_{min} = \argmin\limits_{left_t,right_t}\{|I_{left_{t}}|,|I_{right_{t}}|\}$
        \State $\bullet$ move $|I_{c_{max}}|\cdot \bm{\epsilon_{3}}$ data points in $c_{max}$ with largest error \eqref{eq:partial_objective} to $c_{min}$
        \State
        $\bullet$ determine $\hat{\bm{\w}}_{t}$ by optimizing the BLR function \eqref{eq:reshuffle}
        
            \Else
            \State determine $\hat{\bm{\w}}_{t}$ by optimizing the BLR function \eqref{eq:reshuffle}
            \EndIf
            \State $\hat{\bm{\w}}_{W^k_B} \gets \{\hat{\bm{\w}}_{t},\hat{\bm{\w}}_{W^k_B \setminus t} \}$
        \Else
            \State $\hat{\bm{\w}}_{W^k_B} \gets OptmizeBranchingNode(W^k_B,\bm{\w}^{k-1}_{{\cal C}_{B}(t)})$\Comment{optimization with \textit{\textbf{m}} number of iterations} 
        \EndIf
        
        \State \textbf{return} $\hat{\bm{\w}}_{W^k_B}$
 \EndProcedure
  \end{algorithmic}
  }
\end{algorithm} 
 
 
 
 \subsection{Initialization strategy}\label{subsec:init}
%Looking carefully at the objective function \ref{eq:obj}, it is easy to see that the problem we are dealing with is highly nonconvex and therefore very sensitive to starting points. An appropriate choice of starting points can not only facilitate the training phase but also generate solutions with a better generalization error. 

\textcolor{blue}{It is easy to see that the formulation \ref{eq:obj} is very sensitive to starting points due to is highly nonconvex nature. An appropriate choice of starting points can help the training phase and yield solutions with a better generalization error.}


%To propose a meaningful and useful initialization, we must consider the nature of the problem we are dealing with. A decision tree %is nothing more than a%
%\textcolor{blue}{actually performs a recursive partition of the feature space, hence it divides the data points into subgroups.}

%\textcolor{red}{To devise an effective initialization, we must consider the problem nature: decision trees recursively partition the feature space dividing data into subgroups.}


\textcolor{blue}{The idea for our initialization strategy is to exploit a clustering algorithm to induce a recursive partition of the feature space capable of effectively dividing the data points. Starting from the root node with a single cluster composed of all data points we recursively split the top-level cluster into two sub-clusters so as to have for each leaf node at depth $D$ a distinct cluster.}

\textcolor{blue}{Given $I_t$ as the set of data points falling into branch node $t \in \tau_B$, $I_{left_t}$ and $I_{right_t}$ (i.e. set of data points assigned to its left and right children nodes) are determined by clustering $I_t$ into two clusters. This procedure ensures that clustering at node $t$ is applied only
after having applied it to its anchestor node.}



\textcolor{blue}{Since the initialization procedure may exhibit variability due to the randomness inherent in the clustering method, the initialization procedure is repeated over $v$ trials. In our work, we employ the well-known \textbf{K-means} algorithm \cite{lloyd1982least} with \textit{K-means++} random initialization \cite{arthur2007k}.} 

\textcolor{blue}{For each trial $j = 1,\dots,v$, let $A_{\tau_B\cup\tau_L}^j$ be the assignment of data points to every node of the tree, and $A_{\tau_L}^j \subset A_{\tau_B \cup\tau_L}^j$ be the final partition of all data points into the leaf nodes. At the end of each trial $j$, a silhouette score $Sil(A_{\tau_L}^j)$ is computed on the final partition $A_{\tau_L}^j$ to measure the quality of a given clustering. The assignment with the best silhouette score is selected for the initialization.  In our implementation we consider as silhouette score the Davies-Bouldin index \cite{davies1979cluster} which expresses the average similarity measure of each cluster with its most similar cluster.} 




%Since the clustering is in turn affected by randomness, the initialization procedure is repeated in $v$ trials. For each trial $j = 1,\dots,v$, let $A_{\tau_B,\tau_L}^j$ be the assignment of data points to every node of the tree, and $A_{\tau_L}^j \subset A_{\tau_B,\tau_L}^j$ be the final partition of all data points into the leaf nodes. At the end of trial $j = 1,\dots,v$, a silhouette score, which is a measure of the quality of a given clustering \cite{}, is computed on the final partition $A_{\tau_L}^j$, and it is denoted as $Sil(A_{\tau_L}^j)$. Then the assignment achieving the best silhouette score is the candidate for the initialization. 


 

The general scheme of the initialization procedure is given in Algorithm \ref{alg:init}. It is important to notice that for both the clustering method and silhouette score many alternatives can be considered. 
%In our implementation, the clustering algorithm used is the well-known \textbf{K-means} algorithm with the \textit{K-means++} \textcolor{blue}{initialization CITATIONS}, while the Davies-Bouldin index \cite{} is used as silhouette score. Without entering into details, the Davies–Bouldin index is the average similarity measure of each cluster with its most similar cluster, where similarity is the ratio of within-cluster distances to between-cluster distances. However, for both the clustering method and silhouette score many alternative choices can be considered. 





%To assess the effectiveness of the initialization procedure we present the results of an experiment performed on the Housing dataset (results are similar for the other datasets). The algorithm \ref{} is applied to the training problem of the Housing dataset in a k-fold cross validation with k = 4 and for each fold 20 random clustering are applied for the initialization procedure. Therefore, 80 different training experiments are performed. Then a simple linear regression is fitted to the results of the previous experiments in which the response is the out-of-sample $R^2$ and the predictor variable is the silhouette score associated to each initialization. From the regression results, reported in Figure \ref{fig:statisticainizializzazione}, it is possible to appreciate the high significance and the negative sign of the regression coefficient, showing that a lower silhouette index is higly correlated with a higher out-of-sample $R^2$. Note that in the lower is the Davies-Bouldin score the better is the quality of the clustering.

To assess the effectiveness of our initialization procedure with the selection of the best Davies-Bouldin index, the algorithm \ref{alg:init} and decomposition method are applied to the Housing dataset. A k-fold cross validation with k = 4 is applied and for each fold 20 distinct initialization are generated by the initialization procedure. Then a simple linear regression is fitted to the 80 results where the response is the testing $R^2$ and the predictor variable is the silhouette score associated to each initialization. 

The regression results in Figure \ref{fig:statisticainizializzazione} show a strong negative correlation between the silhouette score and testing $R^2$, as indicated by the high significance and the negative sign of the regression coefficient. Note that the lower is the Davies-Bouldin index the better is the quality of the clustering. 

%From the regression results, reported in Figure \ref{fig:statisticainizializzazione}, it is possible to appreciate the high significance and the negative sign of the regression coefficient, showing that a lower silhouette index is highly correlated with a higher testing $R^2$. Note that in the lower is the Davies-Bouldin score the better is the quality of the clustering.





%The results obtained on the 4 datasets show that the proposed algorithm is able to handle randomized multivariate regression trees well. Nevertheless, a deeper analysis of the solutions found shows that the performance in terms of out-of-sample accuracy is very sensitive to the choice of initial values. This behavior is easily seen looking at the mean and the standard deviation levels of the out-of-sample $R^2$ in the Table \ref{table:confrontoalgo}. The comparison between the  algoritmo proposto and algoritmo proposto+initialization strategy blatantly shows how in all four dataset a clever initialization strategy can make a substantial contribution. 

%To better understand the impact of initialization, we analyse the distribution of instances across leaf nodes. To be more precise, considering each leaf node as a distinct cluster, we use the Davies–Bouldin index as metric for evaluating clustering. The Davies–Bouldin index is the average similarity measure of each cluster with its most similar cluster, where similarity is the ratio of within-cluster distances to between-cluster distances. 
%Taking the Housing dataset as an example (the result is similar with other datasets), the Figure \ref{fig:statisticainizializzazione} summarizes the statistics on fitting the out-of-sample $R^2$ obtained with the proposed algorithm as output variables using as unique regressor variable the Davies–Bouldin index.

\begin{figure}[h]
\centering
\includegraphics[width=0.7\linewidth]{images/statistica_inizializzazione}
\caption{Results obtained on the housing dataset by fitting a linear regression to assess the relation between the testing $R^2$ (response) and the Davies-Bouldin score associated to each initialization (independent variable) generated by our initialization procedure.}
\label{fig:statisticainizializzazione}
\end{figure}




% \begin{algorithm}[H]

% $\bm{Input}:depth \,\bm{D}; \,iterations\, \bm{v}; dataset \bm{X}.\\$ 
% $\bm{Output}:\,dictionary\,with\,instances\,associated\,to\,each\,node\,\bm{dic}^{*}. $
%   \caption{Initialization strategy algorithm}\label{alg:init}
%   \begin{algorithmic}[1]
%     \Procedure{InitializationStrategy}{$\bm{D},\bm{v},\bm{X}$}
%     \State $\bm{dic}^{*} \gets \{\}$ 
%     \State $DBindex^{*} \gets BigM$ \Comment{setting big value for the index}
%     	\For{$ i = 1,...,\bm{v} $}\Comment{loop over the iterations}
%     		\State $j \gets 0$
%     		\State $\bm{dic} \gets \{0: X\}$ \Comment{temporary dictionary}
%     		\While{$ j \leq \bm{D} $}
%     			\State $currentnodes \gets nodesatlevel(j)$ \Comment{list of nodes on}
%     			\State $\qquad \qquad \qquad \qquad \;\,\, \qquad \qquad${which applying clustering algorithm}
%     			\For{$ k\; in\; currentnodes $}
    			
%     			\State $ left_{k} \gets descendant(k,left=\bm{True})$ 
%     			\State $ right_{k} \gets descendant(k,right=\bm{True})$
%     			\State $X_{left_{k}},X_{right_{k}} \gets \textrm{K-means}(X_k,n\_clusters=2)$
%     			\State $\bm{dic}[left_{k}],\bm{dic}[right_{k}] \gets X_{left_{k}},X_{right_{k}} $
%     			\EndFor
    		
%     		\EndWhile
%     	\State $DBindex \gets Davies–Bouldin(\bm{dic})$\Comment{index of last level nodes}
%     	\If{$DBindex < DBindex^{*}$}
%     	      \State $DBindex^{*} \gets DBindex$
%     	      \State $\bm{dic}^{*} \gets \bm{dic}$

%     	\EndIf
    	
%     	\EndFor
%     \State \textbf{return} $\bm{dic^{*}}$
%     \EndProcedure
%   \end{algorithmic}
% \end{algorithm}
 
 
\begin{algorithm}[h]
\caption{Initialization strategy algorithm}
\label{alg:init}
$\bm{Input}:depth \,\bm{D}; \,iterations\, \bm{v}; dataset\, \bm{I}.\\\bm{Output}:\,assignment\,with\,data\,points\,associated\,to\,leaf\,nodes\,{A_{\tau_L}^{j}}^*. $
  
  {\fontsize{10}{12}\selectfont
  \begin{algorithmic}[1]
    \Procedure{InitializationStrategy}{$\bm{D},\bm{v},\bm{I}$}
    
    \State $DB^{*} \gets BigM$ \Comment{setting big value for the index}
    	\For{$ j = 1,...,\bm{v} $}\Comment{loop over the iterations}
    	\State $A_{\tau_B \cup\tau_L}^j \gets \{\{\bm{I}\}\}$ 
    	\State $A_{\tau_L}^j \gets \{\}$
    	
    		\For{$t = 1,...,2^{D-1} $}
    		\State $I_{left_{t}},I_{right_{t}} \gets \textrm{K-means}(I_t,n\_clusters=2)$
    		\State $A_{\tau_B\cup\tau_L}^j \gets A_{\tau_B\cup\tau_L}^j \cup \{I_{left_{t}}\} \cup \{I_{right_{t}}\} $
    		\If{$t \geq 2^{D-2}$}
    		\State $A_{\tau_L}^j \gets A_{\tau_L}^j \cup \{I_{left_{t}}\} \cup \{I_{right_{t}}\} $
    		\EndIf
    		\EndFor
    		
    	\State $DB \gets Davies–Bouldin(A_{\tau_L}^j)$\Comment{index of last level nodes}
    	\If{$DB < DB^{*}$}
    	      \State $DB^{*} \gets DB$
    	      \State ${A_{\tau_L}^{j}}^* \gets A_{\tau_L}^j$

    	\EndIf
    	
    	\EndFor
    \State \textbf{return} ${A_{\tau_L}^{j}}^*$
    \EndProcedure
  \end{algorithmic}
  }
\end{algorithm}
 
\iffalse
\begin{algorithm}[H]
$\bm{Input}:branching\, node\, t ;\,W^k_L\, working \, set;\,depth\, \bm{D};\,training\,data \, \bm{X},\bm{y}.\\$ 
$\bm{Output}:\,optimal\, values\, \hat{\bm{\beta}}_{W^k_L}.$
  \caption{Update Leaf Nodes}\label{alg:updateleaf}
  \begin{algorithmic}[1]
    
    \Procedure{UpdateLeafNode}{$t,W^k_L,\bm{D},\bm{X},\bm{y}$}
    
    \State $ I_{t} \gets IndicesInstances(\bm{X},t)$ \Comment{instances fallen in the node t}
    \If{$D == 1$}\Comment{optimization w.r.t. the children leaf node variables}
        \State $\hat{\bm{\beta}}_{W^k_L} \gets OptmizeLeafNodes(t,I_{t})$ 
                
        \Else \If {$t\; not\; root$}
        	\State $\hat{\bm{\beta}}_{W^k_L} \gets OptmizeLeafNodes(t,I_{t})$ 
        
        \EndIf
        \EndIf
    
        
        \State \textbf{return} $\hat{\bm{\beta}}_{W^k_L}$
 \EndProcedure
  \end{algorithmic}
\end{algorithm}  


\begin{algorithm}[H]
$\bm{Input}:\,branching\,node\,\bm{t};\,training\,data\,\bm{X};\, set\, of\, instances\,fallen\,in\,t\,I_{t};\,\bm{\epsilon_{3}};\,integer\, \bm{FlagBalance}.\\$ 
$\bm{Output}:\,optimal\,values\,\bm{\w}_{t}^{*}. $
  \caption{BalancedLogisticRegression algorithm}\label{shuffle}
  \begin{algorithmic}[1]
    \Procedure{BalancedLogisticRegression}{$t,\bm{X},I_{t},\bm{\epsilon}_{3},\bm{FlagBalance}$}
        \State \Comment{indices of child nodes of t}
        \State $ left_{t} \gets descendant(t,left=\bm{True})$ 
        \State $ right_{t} \gets descendant(t,right=\bm{True})$
        \State $ I_{left_{t}} \gets IndicesInstances(\bm{X},left_{t})$ \Comment{instances fallen on the left}
        \State $ I_{right_{t}} \gets IndicesInstances(\bm{X},right_{t})$ \Comment{instances fallen on the right}
        \State $ label_{I_{t}} \gets label(I_{left_{t}},I_{right_{t}})$\Comment{0-1 encoding for instances fallen into the}
        \State $\qquad \qquad \qquad\qquad\qquad\qquad\quad\:\: ${children}
        \State $\gamma \gets max(|I_{left_{t}}|,|I_{right_{t}}|)\cdot \bm{\epsilon_{3}} $\Comment{number of instances to shuffle}
      \If{$\bm{FlagBalance} != -1 $}
      \If{$\bm{FlagBalance} == 1 $}\Comment{move instances from the most numerous one}
      \State $label_{I_{t}} \gets RandomEncoding(label_{I_{t}},\gamma)$\Comment{random selection}
      \Else \
      \State $label_{I_{t}} \gets DeterministicEncoding(label_{I_{t}},\gamma)$\Comment{selection of instances that weigh more in the} 
      \Statex {\qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad loss of the subtree generated by t}
      \EndIf
      
      \EndIf
      
      \State $\bm{\w}_{t}^{*} \gets BalancedLogistic(I_{t},label_{I_{t}})$
      \State \textbf{return} $\bm{\w}_{t}^{*}$
    \EndProcedure
  \end{algorithmic}
\end{algorithm}
\fi
 

==> sections/old_decomposition.tex <==
%\documentclass[../main.tex]{subfiles}



%\begin{equation}
%\label{eq:formulation}
%\min_{\bm{\w},\bm{\mu}} \frac{1}{|I|}\sum_{i \in I}\sum_{t\in \tau _{L}}\prod_{\ell\in N_{L(t)}}p_{i\ell}(\bm{\w}_{\ell},\mu_{\ell})\;\prod_{r\in N_{R(t)}}(1-p_{ir}(\bm{\w}_r,\mu_r))\cdot(\hat y_{it}(\bm{\w}_{\cdot t},\mu_{t})-y_{i})^{2}
%\end{equation}
\section{A general decomposition algorithm}\label{sec:dec}
 The randomized regression tree model presented in Section ?? is trained by the challenging minimization of the nonconvex function \eqref{eq:formulation1a} with respect to variables $\bm{\w}$ and $\bm{\beta}$. The difficulty of the training problem is not only related to the nonconvexity of \eqref{eq:formulation1a}, but also to the growth of the computational load when the size of the problem increases (number of fetures, number of samples and layers of the tree). A general way to overcome the previous drawbacks is through decomposition algorithms (see e.g., \cite{chang2011libsvm}, \cite{grippo2015decomposition}, \cite{manno2016convergent,manno2018parallel}, and \cite{shalev2011pegasos}), in which the original problem is splitted in a sequence of subproblems, in which only a subset of variables, the so called Working Set, is optimized, while the other are kept fixed to the current value. Decomposition is particularly effective whenever the subproblems have some favorable mathematical structure, as it is the case for the considered formulation \eqref{eq:formulation1}. Indeed, minimizing \eqref{eq:formulation1a} (or equivalently \eqref{eq:formulation1b}) with respect to only the leaf node variables $\bm{\beta}$ (keeping fixed the branching node variables $\bm{\w}$) amounts to a convex linear least squares problem. The strategy of decomposing the original problem so as to preserve the separation between "convex" and "nonconvex" variables, has already proved to be effective in escaping from irrelevant local solutions and in accelerating convergence for other ML models (see e.g., \cite{grippo2015decomposition} and \cite{buzzi2001convergent}). \
 
 For the above reasons, in this section we present a general decomposition algorithmic scheme for solving formulation \eqref{eq:formulation1}, which preserves the separation between the branching node variables and the leaf node variables and may incorporate many different practical versions. Similarly to the decomposition approach devised in \cite{amaldi2021multivariate} for randomized classification trees, the proposed decomposition scheme exploits the intrinsic tree structure of the model by a node-based working set selection procedure.
 
 In the following Section \ref{subsec:scheme}, the general decomposition algorithmic scheme, namely Node Decomposition General Scheme (NDGS), is described in detail, then the asymptotic convergence of NDGS under suitable conditions is stated in Section \ref{subsec:convergence}.
 
 
\subsection{Algorithmic scheme}\label{subsec:scheme}
We consider the following $l_2$ regularized version of formulation \eqref{eq:formulation1}
\begin{equation}\label{eq:obj}
\min_{\bm{\w},\bm{\beta}} E(\bm{\w,\beta}):= \frac{1}{N}\sum_{i \in I}\sum_{t\in \tau _{L}}\prod_{\ell\in A_{L(t)}}p_{i\ell}(\bm{\w}_{\ell})\;\prod_{r\in A_{R(t)}}(1-p_{ir}(\bm{\w}_r))\cdot(\hat y_{it}(\bm{\beta}_t)-y_{i})^{2} + \frac{\lambda_{\bm{\w}}}{2} \|\bm{\w} \|^2+ \frac{\lambda_{\bm{\beta}}}{2} \|\bm{\beta}\|^2,
\end{equation}
where $\lambda_{\bm{\w}},\lambda_{\bm{\beta}}\geq 0$ are the regularization coefficients. Recall that variable $\bm{\w}$ ($\bm{\beta}$) can be rearranged into a matricial form as $\bm{\w} =(\bm{\w}_1,\dots,\bm{\w}_{|\tau_B|}) \in \mathbb{R}^{(p+1) \times |\tau_B|}$ ( $\bm{\beta} =(\bm{\beta}_{1},\dots,\bm{\beta}_{|\tau_L|}) \in \mathbb{R}^{(p+1)\times |\tau_L|}$) where column vector $\bm{\w}_t \in \mathbb{R}^{p+1}$ ($\bm{\beta}_t \in \mathbb{R}^{p+1}$) includes variables associated to branch (leaf) node $t \in \tau_B$ ($t \in \tau_L$). Accordingly, the components of the whole gradient of the objective function $\nabla E(\bm{\w,\beta})$ associated to variables $\bm{\w}$ ($\bm{\beta}$), say $\nabla_{\bm{\w}} E(\bm{\w,\beta})$ ($\nabla_{\bm{\beta}} E(\bm{\w,\beta})$), can be rearranged into matricial form as $\nabla_{\bm{\w}} E(\bm{\w,\beta})=(\nabla_{\bm{\w}_1} E(\bm{\w,\beta}),\dots,\nabla_{\bm{\w}_{|\tau_B|}} E(\bm{\w,\beta})) \in \mathbb{R}^{(p+1)\times |\tau_B|}$ ($\nabla_{\bm{\beta}} E(\bm{\w,\beta})=(\nabla_{\bm{\beta}_1} E(\bm{\w,\beta}),\dots,\nabla_{\bm{\beta}_{|\tau_L|}} E(\bm{\w,\beta})) \in \mathbb{R}^{(p+1)\times |\tau_L|}$). More generally, given a subset of branch (leaf) nodes $J \subseteq \tau_B$ ($J \subseteq \tau_L$) and its complement $\bar J$, variables $\bm{\w}$ ($\bm{\beta}$) can be rearranged as $(\bm{\w}_J,\bm{\w}_{\bar J})$ ($(\bm{\beta}_J,\bm{\beta}_{\bar J})$), and the gradient components associated to $J$ are denoted as $\nabla_J E(\bm{\w,\beta})$. Variables $\bm{\w}$, $\bm{\beta}$, gradient $\nabla E(\bm{\w,\beta})$, and all their subcomponents can be also considered in a flattened vectorial form when needed.
\par 
In the proposed decomposition framework, at each iteration $k$ the Working Set is divided into a branch node index Working Set $W^k_B\subseteq \tau_B$, where each index $t \in W^k_B$ select all variables associated to branch node $t$ (so all elements of column $\bm{\w}_t$), and a leaf node index Working Set $W^k_L \subseteq \tau_L$,  where each index $t \in W^k_L$ select all variables associated to leaf node $t$ (so all elements of column $\bm{\beta}_t$). NDGS proceeds by optimizing, at every iteration, firstly the branching node variables whose indices are in $W^k_B$ ({\bf BN Step}), then the leaf node variables whose indices are in $W^k_L$ ({\bf LN Step}). The NDGS scheme is reported below.  
{\small 
\par\medskip
\hrule
\smallskip
 {\bf NDGS}
\smallskip
\hrule
\par\bigskip\noindent
{Initialization:} determine an initial starting point\par
\centerline{$\bm{\w}^0 =({\bm{\w}^0}_1,\dots,{\bm{\w}^0}_{|\tau_B|})\in \mathbb{R}^{(p+1) \times |\tau_B|}$}
\centerline{$\bm{\beta}^0 =({\bm{\beta}^0}_{1},\dots,{\bm{\beta}^0}_{|\tau_L|})\in \mathbb{R}^{(p+1)\times |\tau_L|} $.}
\par\medskip\noindent Set $k=0$.
\par\smallskip\noindent
{While} the {\it termination test} is not satisfied, choose $W^k_B\subseteq\tau_B, \; W^k_L\subseteq\tau_L$
and perform the following steps.
\par\medskip\noindent
\begin{description}
\item[{\bf BN Step}] {\it (Minimization with respect to the Branching Nodes variables)}
\par\smallskip\noindent
If $ W_{B}^k\equiv \emptyset$ set $\bm{\w}^{k+1}=\bm{\w}^k$, otherwise starting from $(\bm{\w}^{k},\bm{\beta}^k)$, minimize
(exactly or approximately) the function $E(\bm{\w},\bm{\beta})$ in \eqref{eq:obj} with respect to all
$\bm{\w}_t$ for $t\in W^k_B$ determining $\bm{\w}^*_t$ for $t\in W^k_B$, and set the new updated branching node variables as $\bm{\w}_t^{k+1}=\bm{\w}^*_t$ for $t\in W^k_B$ and $\bm{\w}_t^{k+1}=\bm{\w}_t^k$ for $ t\notin W^k_B$, producing $(\bm\w^{k+1},\bm\beta^k)$.


\par\smallskip\noindent
 \item[{\bf LN Step}] {\it (Minimization with respect
to Leaf Nodes variables - Regression)}
\par\smallskip\noindent
If $ W_{L}^k\equiv \emptyset$ set $\bm{\beta}^{k+1}=\bm{\beta}^k$, otherwise starting from $(\bm{\w}^{k+1},\bm{\beta}^k)$, minimize
(exactly or approximately) the function $E(\bm{\w},\bm{\beta})$ in \eqref{eq:obj} with respect to all
$\bm{\beta}_t$ for $t\in W^k_L$ determining $\bm{\beta}^*_t$ for $t\in W^k_L$, and set the new updated leaf node variables as $\bm{\beta}_t^{k+1}=\bm{\beta}^*_t$ for $t\in W^k_L$ and $\bm{\beta}_t^{k+1}=\bm{\beta}_t^k$ for $ t\notin W^k_L$, producing $(\bm\w^{k+1},\bm\beta^{k+1})$.

\end{description}
\par\smallskip  Set $k=k+1$.
\par\medskip\noindent
 {End While}
 \smallskip
\hrule
 \medskip
 
 }
%  %%%%%%%%%%%
% \begin{algorithm}[H]  \caption{Decomposition General Scheme (DGS)}\label{alg:DGS}
% \Statex {\bf initialization}: determine an initial starting point\\
% \centerline{$\bm{\w}^0 =({\bm{\w}^0}^T_1,\dots,{\bm{\w}^0}^T_{2^D-1})\in \mathbb{R}^{(p+1)(2^{D}-1)},$}
% \centerline{$\bm{\beta}^0 =({\bm{\beta}^0}^T_{2^D},\dots,{\bm{\beta}^0}^T_{2^{D+1}})^T\in \mathbb{R}^{(p+1)2^{D}} $,}\\
% set $k=0$.\\
%  % \begin{algorithmic}[1]
    
%     \While {\it termination test}
%         \State ({\it working set selection}) select $W^k_B\subseteq\tau_B, \; W^k_L\subseteq\tau_L$
%         \State {\bf BN Step} {\it (Minimization with respect to the Branching Nodes parameters)}
%          Starting from $(\bm{\w}^{k},\bm{\beta}^k)$, minimize
%         (exactly or approximately) the function $E$ with respect to all
%         $\bm{\w}_j$ for $j\in W^k_B$ determining $\bm{\w}^*_j$ for $j\in W^k_B$, and set the new updated branching nodes variables as $\bm{\w}_j^{k+1}=\bm{\w}^*_j$ for $j\in W^k_B$ and $\bm{\w}_j^{k+1}=\bm{\w}_j^k$ for $ j\notin W^k_B$.
%         \State {\bf LF Step} {\it (Minimization with respect to Leaf Nodes parameters - Regression)} Starting from $(\bm{\w}^{k+1},\bm{\beta}^k)$, minimize (exactly or approximately) the function $E$ with respect to all $\bm{\beta}_j$ for $j\in W^k_L$ determining $\bm{\beta}^*_j$ for $j\in W^k_L$, and set the new updated leaf nodes variables as $\bm{\beta}_j^{k+1}=\bm{\beta}^*_j$ for $j\in W^k_L$ and $\bm{\beta}_j^{k+1}=\bm{\beta}_j^k$ for $ j\notin W^k_L$.
%     \EndWhile

% %  \end{algorithmic}
% \end{algorithm}  
% %%%%%%%%%%%

NDGS is very general and may encompass many different versions by specifying: the termination test (which may be related to a tolerance on the norm of the gradient vector of  $E(\bm{\w,\beta})$ or to a maximum number of main iterations), the working set selection rule, the way to update the branching node variables at {\bf BN Step}, and the way to update the leaf node variables at {\bf LN Step}.
The only strict requirement is to maintain the separation between branching node and leaf node variables to exploit the favorable structure of the loss function $E(\bm{\w,\beta})$, which is a (strictly for $\lambda_{\beta}>0$) convex quadratic problem with respect to variables $\bm{\beta}_t$ for $t \in  W_{L}^k$. Therefore, the minimization in the {\bf LN Step} (regression) amounts to solve a linear least squares problem, whose global minimizer can be determined exactly or approximately via efficient methods. Conversely, in the {\bf BN Step} a non convex problem is solved (notice that $E(\bm{\w,\beta})$ is not convex with respect to the branching node variables $\bm{\w}$), so, in general, only approximate solutions of the minimization problem can be obtained.  \par
Another requirement is to retain a ``node decomposition" structure, i.e., to consider all the variables associated to a certain node whenever such a node is inserted in the working set. In principle, one might consider Working Sets including only a subset of variables associated to a node of the tree, but these kinds of scheme will be not considered here. Notice also that, while a sequential ordering between {\bf BN Step} and {\bf LN Step} is formally imposed in the scheme, the possibility of setting $ W_{B}^k\equiv \emptyset$ or $ W_{L}^k\equiv \emptyset$ for any $k$ implies no actual ordering between the two minimization steps.   \par 
One possible NDGS version is obtained if $W_{B}^k\equiv \tau_{B}$ and $W_{L}^k\equiv \tau_{L}$ for all $k$. Then, the algorithm results in an alternating minimization with respect to two blocks, one associated to the branching node variables, and the other to the leaf node variables. Otherwise, one may consider a version in which at each main iteration only variables associated to a single node are optimized (either $W_{B}^k:=\{t\} \mbox{ with } t \in \tau_{B}, W_{L}^k\equiv \emptyset$, or $ W_{B}^k\equiv \emptyset, W_{L}^k:=\{t\} \mbox{ with } t \in \tau_{L}$). These two versions correspond to two opposite strategies, the former characterized by the lowest decomposition level, while the latter by the highest decomposition level. The generality of NDGS allows the design of many algorithms in between the two previous strategies. \par In Section \ref{subsec:implementation} we will present a version of NDGS, namely algorithm DECO, which implements a decomposition particularly suited for the structure of the tree and of the objective function \eqref{eq:obj} and that, combining a clutering-based initialization with a controlled reshuffling heuristic, is able to produce good regression models in relatively short training times.  \par
In the next section we will state the asymptotic convergence of NDGS.
\subsection{Asymptotic convergence of NDGS}\label{subsec:convergence}
In this section the asymptotic convergence of NDGS is discussed. The detailed convergence analysis, which is an adaptation of the one reported in \cite{grippo2015decomposition} for a training algorithm for multi-layer perceptrons, and based on the theory developed in \cite{grippof1999globally}, is described in the Electronic Companion \ref{sec:ec-1}.\par 
First, to establish convergence of NDGS towards stationary points, we have to assume that $\lambda_{\bm\w},\lambda_{\bm\beta}>0$, so that the objective function \eqref{eq:obj} is continuous and coercive and the problem of minimizing it is well defined. Indeed, all its level sets, defined for given $(\bm\w^0,\bm\beta^0)$ as ${\cal L}_0:=\{(\bm\w,\bm\beta) \in \mathbb{R}^{(p+1) \times (|\tau_B|+|\tau_L|)} :E(\bm\w,\bm\beta)\leq E(\bm\w^0,\bm\beta^0)\}$, are compact and then \eqref{eq:obj} admits a global minimizer. \par 
Now to guarantee convergence, three conditions must be enforced, which are relevant both from a theoretical and a practical point of view. The conditions, which are formally stated in the Electronic Companion \ref{subsec:ec-1-ndgs} and whose rationale is described below, assume that NDGS generates an infinite sequence $\{(\bm\w^k,\bm\beta^k)\}$.
%%%%%%%%%%%%%%%%%%%%
% For the following conditions we introduce some intuitive and useful notations.
%We denote with $\nabla_{\bm\w_j}E(\cdot)$, $\nabla_{\bm\beta_i}E(\cdot)$, $\nabla_{W_{B}}E(\cdot)$, and $\nabla_{W_{L}}E(\cdot)$, the subvectors of the gradient $\nabla E(\cdot)$ of \eqref{eq:obj} associated to the components of, respectively, the branching node variables in $\bm\w_j$ with $j \in \tau_B$, the leaf node variables in $\bm\beta_i$ with $i \in \tau_{L}$, all the branching node variables whose index of the corresponding node is in $W_{B}$, and all the leaf node variables whose index of the corresponding node is in $W_{L}$. More generally, given any non-empty subset of branching node indices $J\subseteq \tau_B$, the components vector $\bm\w \in  \mathbb{R}^{(p+1)(2^{D}-1)}$ can be rearranged as $\bm\w=(\bm\w_J^T,\bm\w_{\bar J}^T)^T$, where $\bm\w_J$ is the subvector with components associated to all the variables corresponding to branching nodes in $J$, while subvector $\bm\w_{\bar J}$ is made up of the remaining ones. Analogously, for a non-empty subset of leaf node indices $I\subseteq \tau_L$, the components vector $\bm\beta \in \mathbb{R}^{(p+1)2^{D}}$ can be rearranged as $\bm\beta=(\bm\beta_{I}^T,\bm\beta_{\bar I}^T)^T$. $\nabla_{J}E(\cdot)$ and $\nabla_{I}E(\cdot)$ are the subvectors of the gradient $\nabla E(\cdot)$ with components of, respectively, $\bm\w_j$ with $j \in J$, and $\bm\beta_i$ with $i \in I$.
%%%%%%%%%%%%%%%%%%%%
The three conditions are as follows:
\begin{itemize} 
    \item 
    \begin{condition}\label{con:1} 
    Each branching or leaf node is periodically inserted in the working set. \end{condition} 
     \item 
     \begin{condition}\label{con:2} 
     In the {\bf BN Step}: (i) $E(\bm\w^{k+1},\bm\beta^k)\leq E(\bm\w^{k},\bm\beta^k)$, i.e. the partial update $(\bm\w^{k+1},\bm\beta^{k})$ is not worse than $(\bm\w^{k},\bm\beta^{k})$ in terms of objective function value; (ii) for an infinite subsequence $K$ in which the index $t \in \tau_B$ of a given block of variables $\bm\w_t$ is inserted in the branch nodes Working Set $W_{B}^k, k\in K$, then $\lim\limits_{k \to \infty. k \in K} \|\bm\w_t^{k+1}-\bm\w_t^k\|=0$, i.e.  the distance between successive iterates tends to zero; (iii) it holds $\lim\limits_{k \to \infty. k \in K} \nabla_{\bm\w_t}E(\bm\w^{k},\bm\beta^k)=0$, i.e., at least in the limit, the first order optimality conditions are satisfied with respect to the $w_t$ gradient components.
     \end{condition} 
     \item 
     \begin{condition}\label{con:3}
     In the {\bf LN Step}: (i) $E(\bm\w^{k+1},\bm\beta^{k+1})\leq E(\bm\w^{k+1},\bm\beta^k)$, i.e. the partial update $(\bm\w^{k+1},\bm\beta^{k+1})$ is not worse than $(\bm\w^{k+1},\bm\beta^{k})$ in terms of objective function value; (ii) for every $t \in \tau_L$ and for an infinite subsequence $K$ in which the index $t$ of a given block of variables $\bm\beta_t$ is inserted in the leaf nodes Working Set $W_{L}^k, k \in K$, then $\lim\limits_{k \to \infty. k \in K} \nabla_{\bm\beta_t}E(\bm\w^{k+1},\bm\beta^{k+1})=0$, i.e. at least in the limit, a convergent algorithm is applied.
     \end{condition}
\end{itemize}
\textsc{Condition} \ref{con:1} can be easily ensured in a constructive matter. Notice also that \textsc{Condition} \ref{con:2} and \ref{con:3} are similar, but the latter is less restrictive than the former. Indeed, due to the strict convexity (recall $\lambda_{\bm\beta}>0$) of the optimization problem related to the {\bf LN Step}, the requirement of the distance between successive iterates tending to zero (analogous to point (ii) of Condition \ref{con:2}) is automatically ensured (see Electronic Companion \ref{subsec:ec-1-ndgs} for details). \par 
Now it is possible to state the following asymptotic convergence result.
\begin{proposition}\label{prop:prop1}
Suppose that NDGS generates an infinite sequence
 $\{(\bm\w^k, \bm\beta^k)\}$ and that Conditions \ref{con:1},  \ref{con:2} and \ref{con:3}  are
 satisfied. Then:
\begin{description}
 \item[(i)] the sequence $\{(\bm\w^k, \bm\beta^k)\}$ has limit points;
 \smallskip
\item[(ii)] the sequence $\{E(\bm\w^k, \bm\beta^k)\}$ converges to a
limit; \smallskip
 \item[(iii)] $\lim\limits_{k\to\infty}\|\bm\w^{k+1}-\bm\w^k\|=0;$
\smallskip
 \item[(iv)] $\lim\limits_{k\to\infty}\|\bm\beta^{k+1}-\bm\beta^k\|=0;$
\smallskip
 \item[(v)] every limit point of $\{(\bm\w^k,
\bm\beta^k)\}$ is a stationary point of $E(\bm\w,
\bm\beta)$ in \eqref{eq:obj}.
\end{description}
\qedblack
\end{proposition}
The proof of Proposition \ref{prop:prop1}, together with two technical lemmas required in the proof, are reported in the Electronic Companion \ref{subsec:ec-1-ndgs}.

% \par 


%\end{document}


==> sections/proposed_algorithm.tex <==
%\documentclass[../main.tex]{subfiles}

\section{The proposed algorithm}\label{sec:algorithm}
  


\subsection{A suitable algorithm vs. a simple decomposition scheme }
In order to assess the need of a more complex algorithm  we compare the simple decomposition scheme with our proposed algorithm in a synthetic dataset. 








%hildren nodes $I_{left_t}$ and $I_{right_t}$. If the imbalance between the data of the child nodes does not exceed the threshold $\epsilon_1$ we optimize the variables $a_t$ and $\mu_t$ through a generic solver, otherwise we check if the imbalance is greater than the second threshold $\epsilon_2$. If the imbalance is higher than the threshold $\epsilon_2$ we apply the procedure \textit{BalancedLogisticRegression} with reshuffling, otherwise the procedure \textit{BalancedLogisticRegression} is applied without reshuffling. Next if the children of the node $t$ are leaf nodes we proceed with the optimization of the predictor variables $a_{left_t},a_{right_t},\mu_{left_t},\mu_{right_t}$ by means of \textit{OptmizeLeafNodes.}}

% \textcolor{red}{The \textit{BalancedLogisticRegression} procedure is divided in two phases: the labeling encoding of the instances fallen in the two children nodes and the balanced logistic regression.
% The first step depends on the value of the variable $\bm{r}$, in case a shuffling of instances is necessary (i.e. $\bm{r}!=1$) either random (i.e.$\bm{r}=1$) or deterministic (i.e. $\bm{r}!=0$) shuffling will be applied. Next a logistic regression is computed where adjusted weights associated with classes (class 0 for the left branch 1 for the right one) are imposed. The weights are inversely proportional to class frequencies in the input data. }

% \textcolor{red}{In the experiments for the computation of the balanced logistic regression we used the \texttt{scikit learn} package with the default settings where the solver is \textit{lbfgs} and $l_2$ penalty is applied with the default value of inverse of regularization strength. Whereas the procedure \textit{OptimizedBranchingNode} simply optimizes the logistic regression without any regularization or balance induced, using the SLSQP solver in \texttt{scipy.optimize} package in tandem with \texttt{numba}. For the \textit{OptmizeLeafNodes} we used different optmization techniques depending on the regularization term applied in the leaf nodes. Indeed in the case of $l_2$ regularization or absence of regularization we find the least-squares solution by means of the command \texttt{scipy.sparse.linalg.lsqr} in the scipy sparse linear algebra package  \texttt{scipy.sparse}. In the case of the $l_0$ concave approximation we use the SLSQP solver in \texttt{scipy.optimize} package in tandem with \texttt{numba} } 

% \iffalse
% \begin{algorithm}[H]
% $\bm{Input}: depth \,\bm{D}; training\,data \, \bm{X}, \bm{y}; starting\,values \,\bm{a}, \bm{\mu};\,max\,iterations\,\bm{M};\\ \,mini\,iterations\,\bm{m};\,\bm{\epsilon_{1}};\,\bm{\epsilon_{2}};\,\bm{\epsilon_{3}};\,\bm{\gamma};\,integer\,\bm{r}.\\$ 
% $\bm{Output}:\,optimal\, values\, \bm{a^{*}},\,\bm{\mu^{*}}.$
%   \caption{Decomposition algorithm}\label{Decomposition}
%   \begin{algorithmic}[1]
    
%     \Procedure{Decomposition}{$\bm{D},\bm{X},\bm{y},\bm{a},\bm{\mu},\bm{\epsilon_{1}},\bm{\epsilon_{2}},\bm{\epsilon_{3}},\bm{\gamma},\bm{r}$}
%       \State $ boolean\,\bm{condition}  \gets \bm{True} $
%       \State $\bm{a}^{*},\bm{\mu}^{*} \gets \bm{a},\bm{\mu}.$
%       \State $error_{best} \gets loss(\bm{a}^{*},\bm{\mu}^{*},\bm{X},\bm{y}).$
%       \State $i \gets 1.$
%       \While{$ i < \bm{M}\,and\,\bm{condition} $}
%         \For{$ t = 1,...,2^{\bm{D}}-1 $}\Comment{loop over the branching nodes}
%         \State \Comment{indices of child nodes of t}
%         \State $ left_{t} \gets descendant(t,left=\bm{True})$ 
%         \State $ right_{t} \gets descendant(t,right=\bm{True})$
%         \State $ I_{t} \gets IndicesInstances(t)$ \Comment{instances fallen in the node t}
%         \State $ I_{left_{t}} \gets IndicesInstances(left_{t})$ \Comment{instances fallen on the left}
%         %\ifthenelse{}{}{}
%         \If{$\frac{|I_{left_{t}}|}{|I_{t}|} \leq \bm{\epsilon_{1}}$ or\, $\frac{|I_{left_{t}}|}{|I_{t}|} \geq 1 - \bm{\epsilon_{1}}$ }\Comment{unbalanced }
%         \State $ \qquad\qquad\qquad\qquad\qquad \qquad\qquad\qquad\qquad ${instances in children}
%             \If{$\frac{|I_{left_{t}}|}{|I_{t}|} \leq \bm{\epsilon_{2}}$ or\, $\frac{|I_{left_{t}}|}{|I_{t}|} \geq 1 - \bm{ \epsilon_{2}}$}\Comment{worse unbalance }
%         \State $\bm{a}_{\cdot t}^{*},\bm{\mu}_{t}^{*} \gets $\textsc{BalancedLogisticRegression}$(t,\bm{\epsilon_{3}},\bm{r})$
%             \Else
%             \State $\bm{a}_{\cdot t}^{*},\bm{\mu}_{t}^{*} \gets $\textsc{BalancedLogisticRegression}$(t,\bm{\epsilon_{3}},\bm{r}=-1)$
%             \EndIf
%         \Else
%             \State $\bm{a}_{\cdot t}^{*},\bm{\mu}_{t}^{*} \gets OptmizeBranchingNode(t,\bm{m})$\Comment{optimization w.r.t. the variables in t} \State $\qquad \qquad \qquad\qquad \qquad\qquad\qquad \qquad\:\,\, $
%             \State $\qquad \qquad \qquad\qquad \qquad$ {with a maximum number of iterations } 
%         \EndIf
%         \If{$D == 1$}\Comment{optimization w.r.t. the children leaf node variables}
%         \State $\bm{a}_{\cdot (left_{t}, right_{t})}^{*},\bm{\mu}_{(left_{t}, right_{t})}^{*} \gets OptmizeLeafNodes(t)$ 
                
%         \Else \If {$t\; not\; root$}
%         	\State $\bm{a}_{\cdot (left_{t}, right_{t})}^{*},\bm{\mu}_{(left_{t}, right_{t})}^{*} \gets OptmizeLeafNodes(t)$ 
        
%         \EndIf
%         \EndIf
%         %\If{$(left_{t}, right_{t}) \in %\tau_{L}$}\Comment{the children nodes are leaf nodes}
%         %\State \Comment{optimization w.r.t. the children %leaf node variables}
%         %\State $\bm{a}_{\cdot (left_{t}, %right_{t})}^{*},\bm{\mu}_{(left_{t}, right_{t})}^{*} %\gets OptmizeLeafNodes(t)$
%         %\EndIf
%         \If{$loss(\bm{a},\bm{\mu},\bm{X},\bm{y})< error_{best}$}
%         \State $error_{best} \gets loss(\bm{a},\bm{\mu},\bm{X},\bm{y})$.
%         \State $\bm{a}^{*},\bm{\mu}^{*} \gets \bm{a},\bm{\mu}$.
%         \EndIf
%         %\State \texttt{left_{t} = descendant(t,right=\bm{True})}
%         \EndFor
% 	  \State $\bm{\epsilon_{1}},\,\bm{\epsilon_{2}},\,\bm{\epsilon_{3}} \gets \bm{\gamma}\cdot\bm{\epsilon_{1}},\,\bm{\gamma}\cdot\bm{\epsilon_{2}},\,\bm{\gamma}\cdot\bm{\epsilon_{3}}$.
%       \EndWhile\label{Decompositiondwhile}
%       \State \textbf{return} $\bm{a}^{*},\bm{\mu}^{*}$
%     \EndProcedure
%   \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}[H]
% $\bm{Input}:\,branching\,node\,\bm{t};\,training\,data\,\bm{X};\, set\, of\, instances\,fallen\,in\,t\,I_{t};\,\bm{\epsilon_{3}};\,integer\, \bm{r}.\\$ 
% $\bm{Output}:\,optimal\,values\,\bm{a}_{\cdot t}^{*},\,\bm{\mu}_{t}^{*}. $
%   \caption{BalancedLogisticRegression algorithm}\label{shuffle}
%   \begin{algorithmic}[1]
%     \Procedure{BalancedLogisticRegression}{$t,\bm{X},I_{t},\bm{\epsilon}_{3},\bm{r}$}
%         \State \Comment{indices of child nodes of t}
%         \State $ left_{t} \gets descendant(t,left=\bm{True})$ 
%         \State $ right_{t} \gets descendant(t,right=\bm{True})$
%         \State $ I_{left_{t}} \gets IndicesInstances(\bm{X},left_{t})$ \Comment{instances fallen on the left}
%         \State $ I_{right_{t}} \gets IndicesInstances(\bm{X},right_{t})$ \Comment{instances fallen on the right}
%         \State $ label_{I_{t}} \gets label(I_{left_{t}},I_{right_{t}})$\Comment{0-1 encoding for instances fallen into the}
%         \State $\qquad \qquad \qquad\qquad\qquad\qquad\quad\:\: ${children}
%         \State $\gamma \gets max(|I_{left_{t}}|,|I_{right_{t}}|)\cdot \bm{\epsilon_{3}} $\Comment{number of instances to shuffle}
%       \If{$\bm{r} != -1 $}
%       \If{$\bm{r} == 1 $}\Comment{move instances from the most numerous one}
%       \State $label_{I_{t}} \gets RandomEncoding(label_{I_{t}},\gamma)$\Comment{random selection}
%       \Else \
%       \State $label_{I_{t}} \gets DeterministicEncoding(label_{I_{t}},\gamma)$\Comment{selection of instances that weigh more in the loss of the subtree generated by t}
%       \EndIf
      
%       \EndIf
      
%       \State $\bm{a}_{\cdot t}^{*},\bm{\mu}_{t}^{*} \gets BalancedLogisticRegression(I_{t},label_{I_{t}})$
%       \State \textbf{return} $\bm{a}_{\cdot t}^{*},\bm{\mu}_{t}^{*}$
%     \EndProcedure
%   \end{algorithmic}
% \end{algorithm}
% \fi

 


%\end{document}
